ARIS: Authentication for Real-Time IoT Systems

Efficient authentication is vital for IoT applications with stringent minimum-delay requirements (e.g., energy delivery systems). This requirement becomes even more crucial when the IoT devices are battery-powered, like small aerial drones, and the efficiency of authentication directly translates to more operation time. Although some fast authentication techniques have been proposed, some of them might not fully meet the needs of the emerging delay-aware IoT. In this paper, we propose a new signature scheme called ARIS that pushes the limits of the existing digital signatures, wherein commodity hardware can verify 83,333 signatures per second. ARIS also enables the fastest signature generation along with the lowest energy consumption and end-to-end delay among its counterparts. These significant computational advantages come with a larger storage requirement, which is a highly favorable trade-off for some critical delay-aware applications. These desirable features are achieved by harnessing message encoding with cover-free families and special elliptic curve based one-way function. We prove the security of ARIS under the hardness of the elliptic curve discrete logarithm problem in the random oracle model. We provide an open-sourced implementation of ARIS on commodity hardware and 8-bit AVR microcontroller for public testing and verification.

==> ARIS Arxiv/Schemes.tex <==



\section{Proposed Scheme}\label{sec:proposed}

\eda~leverages the  homomorphic property of its underlying ECDLP-based one-way function, which is due to the exponent product of powers property, to achieve (polynomially-bounded)  multiple-time signatures from the one-time signature scheme proposed in \cite{Reyzin2002}, with   more compact signatures.  More specifically, in \eda, the private key consists of $ t $ randomly generated values $ x_i $ (generated using a $ \kappa $ bit seed $ z $) and the corresponding public key consists of all $ Y_i \gets  x_i P $ for  $ i \in \{1,\dots,t\} $.   

 To sign a message,  the signer obtains $ k $ indexes $ (i_1, \dots, i_k) $ by hashing the message (and a random input), uses the indexes  $ (i_1, \dots, i_k) $ to retrieve the corresponding private key elements (i.e., $  x_{i_j}$ where $ j \in \{1,\dots,k\} $) and sums them along with a one-time randomness $ r $.  The signature consists  of $ s $ and $ h $, which is obtained by applying the hash function $ \hash_2(\cdot) $  on $ R $,  that is computed as the output of applying the  one-way  function 
%\myedit{say in the first parag. above we use scalar-mul as a fast and compact ECDLP-based onw-way function, and avoid repeating here twice, by saying just scalar multiplication}
 on the one-time randomness $ r $.  
 
 Verification takes place by computing the summation of  the corresponding public key elements  (i.e., $  Y_{i_j}$)  and their subtraction from the output of the ECDLP-based one-way function applied on  $ s $.  The verifier outputs \emph{valid} if the subtraction  yields the same value of $ R $ as computed in the signature generation. Additionally, \eda~uses the BPV method in~\cite{BPV:basepaper:1998} to convert  an EC scalar multiplication to only $ k $ (where  $ k =18 $ or $k=28$ for our proposed parameter sets) EC point additions with the cost of storing a small, constant-size table.
 
%The idea behind the proposed scheme is to leverage the multiplicative property of RSA trapdoor permutation function (Definition \ref{RSA-perm}) to transform one-time HORS~\cite{Reyzin2002} signatures into an (practically) unbounded time signature. Specifically, our private key consists of $ t $ randomly generated values $ s_i $ (that can be deterministically generated with a seed) and the corresponding public key consists of all $ V_i \gets (\RSAEval((N,e),s_i))^{-1} \mod N $ where $ i \in \{1,\dots,t\} $. To sign a message, we compute $\gamma$ by combining a subset of $k$ selected one-time signature components (i.e., $s_i$'s whose indexes $(i_1,\ldots,i_k)$ are obtained from the message hash output, as in HORS) along with a  one-time randomness  $r $ to prevent their disclosure. Recall that the release of the private key components with each signature is the main reason that HORS is a one-time signature. We then compute $R\gets\RSAEval((N,e),r) $ and set the \eda~signature as $ \sigma = (R,\gamma) $. Upon receiving the signature, the verifier first multiplies the subset of corresponding public keys from $PK$ and calculates $\Gamma$. The verifier checks $ R = \RSAEval((N,e),\gamma) \cdot {\Gamma} $, and returns valid (1) if it holds; otherwise returns invalid (0).

%{\em Main Idea}: The idea behind the proposed scheme is to leverage the homomorphic  property of RSA trapdoor permutation functions (Definition \ref{RSA-perm}) to transform a subset-resilient one time signature (i.e., HORS \cite{Reyzin2002}) into an (practically) unbounded time signature. More specifically, the private key consists of $ t $ randomly generated values $ s_i $ (that can be deterministically generated with a seed) and the corresponding public key consists of all $ V_i \gets (\RSAEval(s_i))^{-1} \mod N $ where $ i \in \{0,\dots,t\} $. To sign a message we aggregate one-time signature components (which are the elements of the user's private key) along with a  one-time randomness  $r $ to prevent their disclosure (the release of the private key components with each signature is the main reason that HORS is a one-time signature). We then compute $R\gets\RSAEval(r) $, incorporate $r$, along with the private key components, to calculate $\sigma$, and output the signature as $ \sigma = (R,\gamma) $. Upon receiving the signature, the verifier first multiplies the subset of corresponding public keys from $PK$ and calculates $\Gamma$. Then, it checks if $ R = \RSAEval(\gamma) \cdot {\Gamma} $ outputs valid and otherwise, invalid.


% We require two instantiations of Pseudo Random Functions (PRF). PRF is a polynomial-time computable function which generates  outputs that are indistinguishable from uniform random for a polynomial time distinguisher. We define two different PRF instantiations to be used in our schemes as  $\ensuremath{PRF_1}:\zo^{*} \rightarrow D_i$ and $\ensuremath{PRF_2}:\zo^{*} \rightarrow D_i$. We also define two hash functions (which are treated as random oracles in our scheme) as    $ H_1:\{0,1\}^* \rightarrow \{0,1\}^{l_1}$ and  $ H_2:\{0,1\}^* \rightarrow \{0,1\}^{l_2}$ where $ l_1  $ will be defined based on the security  parameters $ \kappa $ and $ l_2  = k \cdot \log_2 t $ for $ k  $ and $ t $ as \hors~parameters.


Our scheme consists of the following algorithms.  
\noindent  $\underline{(\sk,\pk)\as \edakg(1^{\kappa})}$: Given the security parameter $ \kappa  $, this algorithm selects parameters $ (t,k) $  such that $     \binom{t}{k} \geq 2^\kappa$ and $z  \Ra \Zp $ and works as follows.
 \begin{enumerate} 
   
 \item Compute $ x_i \gets \prf_1(z,i)$  and  $ Y_i  \gets x_iP \mod  q $ for $ i\in \{1,\dots,t\} $ and set $ \mathbf{Y} \gets \{Y_i\}_{i=1 } ^{ t} $.
 \item Compute $ r_i \gets \prf_2(z,i)$  and  $ R_i  \gets r_iP \mod  q  $ for $ i\in \{1,\dots,t\} $ and set $ \mathbf{R} \gets \{R_i\}_{i=1 } ^{ t} $. 
 	\item Output    $   pk \gets   \mathbf{Y} $ and  $\sk \gets (z,\mathbf{R})   $ as the public key and private key, respectively.
 \end{enumerate}

%\footnote{Note that $ V_i, i=1,\ldots,t $ are relatively prime to $N$ with an overwhelming probability, and therefore the inversion fails only with a negligible probability in terms of $\kappa$}
\noindent $\underline{\sigma\as \edasig(m,\sk)}$: Given a message $ m\in \{0,1\}^* $ to be signed, this algorithm works as follows.
\begin{enumerate}
	\item Compute $ (i'_1,\dots,i'_k) \gets \hash_1(m,z)$ where $ |i'_j| \leq |t| $ for $ j\in \{1,\dots,k\} $.
	\item Compute $ r_{i'} \gets \prf_2(z,i'_j)$  for $ j\in \{1,\dots,k\} $, set $ r \gets \sum_{i'=1}^{k} r_{i' } \mod p $.
	\item Retrieve $ R_{i'} \gets \mathbf{R}[i'_j] $  for $ j\in \{1,\dots,k\} $,  compute $ R \gets  \sum_{i'=1}^{k} R_{i'}\mod  q $ and $ h\gets \hash_2(R) $.
	\item Compute $ (i_1,\dots,i_k) \gets \hash_3(m,h)$ (where $ |i_j| \leq |t| $)  and $ x_{i}\gets \prf_1(z,i_j)$  for $ j\in \{1,\dots,k\} $. 
	\item  Compute  $ s \gets r  - \sum_{i=1}^{k}x_{i} \mod p $ and output $ \sigma \gets (s,h) $.
 	
%	\item Generate $ r \as PRF_2{(z ||c)}$ and  $R \as \RSAEval(\pk', r)$ and increment the counter $ c\as c+1$.
%	\item Compute $h \as H_1(R)$ and $(i_1,\ldots,i_k) \as H_2(m||h)$ where    $\{i_j\}_{j=1}^{k} \in [1,t]$ and $ |i_ j|  = \log_2 t $.
%	\item Generate $s_{i_j} \as PRF_1({z||i_j)}$ for $j = 1,\ldots,k$ and compute $\gamma = (\prod_{j=1}^{k} s_{i_j}) \cdot r \mod N$ to output the signature as  $\sigma=(\gamma,h)$.
\end{enumerate}


 \noindent $\underline{\zo\as \edaver(m,\sigma,\pk)}$: Given a message-signature pair $  (m,\sigma) $ and $ pk  $, this algorithm works as follows.
 \begin{enumerate}
 	\item Parse $ (s,h) \gets   \sigma $ and compute $(i_1,\ldots,i_k) \as \hash_3(m,h)$,   where $ |i_j| \leq |t| $ for $ j\in \{1,\dots,k\} $.
 	\item Retrieve   $ Y_i\gets \mathbf{Y} [i_j] $ for $ j\in \{1,\dots,k\} $) and set $ Y \gets \sum_{i=1}^{k} Y_i \mod q  $.
 	\item Compute $ R' \gets sP + Y  \mod q  $ and check if $ \hash_2(R')  = h$ holds output \emph{valid}, and \emph{invalid } otherwise. 

 \end{enumerate}

%
%
%
%\begin{algorithm}[h]
%	\caption{Compact Energy and Delay-aware Authentication (\eda) - RSA instantiation (\edaRsa)}\label{alg:FAHOW_RSA}
%	\hspace{5pt}
%	\begin{algorithmic}[1]
%		
%		\Statex   $\underline{(\sk,\pk)\as \edakg(1^{\kappa})}$: Executed offline (once).
%%%		\vspace{3pt}
%		\State $(t,k)$ are \hors~parameters as in Definition \ref{def-HORS}.
%		\State $(\sk',\pk') \leftarrow \RSAGen(1^{\kappa})$, where $\sk' = (N,d)$ and $\pk' = (N,e)$.
%		\State $s_i\as \PRF{z\norm{i}0}$, $i = 1,\ldots,t$ where $z\Ra\zo^{\kappa}$
%		\State $V_i \gets \RSAEval(\pk', s_i)$,   $i = 1,\ldots,t$\footnote{We note that we assume that $ V_i $s are relatively prime to $ n  $ with a high probability.} and set a counter $ c \gets 0. $
%		\State $\sk = z $, $\pk = (V_1^{-1},\ldots,V_t^{-1})$ and public parameters $ params = (\pk',t,k) $.
%	\end{algorithmic}
%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex $\underline{\sigma\as \edasig(m,\sk)}$: Given a message $m\in \zo^{*}$, compute its signature as follows:
%		\vspace{3pt}
%		\State $r \as \PRF{z \norm{c}1}$, $R \as \RSAEval(r)$, where $c$ is a counter starting from $t+1$.
%		\State $h \as H_1(R)$
%		\State $(i_1,\ldots,i_k) \as H_2(m||h)$, where $\{i_j\}_{j=1}^{k} \in [1,t]$ and $  i_j \leq t $.
%		\State $s_{i_j} \as \PRF{z\norm{i_j}0}$, $j = 1,\ldots,k$.
%		\State $\gamma = (\prod_{j=1}^{k} s_{i_j}) \cdot r$ mod $n$
%		\State $\sigma=(\gamma,h)$.
%	\end{algorithmic}
%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex $\underline{\zo\as \edaver(m,\sigma,\pk)}$: Given $m\in \zo^{*}$, verify its signature $\sigma=(\gamma,h)$ under $\pk = (V_1^{-1},\ldots,V_t^{-1})$ as follows:
%		\vspace{3pt}
%		\State $(i_1,\ldots,i_k) \as H_2(m||h)$ where $ i_j \leq t$  for $ j \in[1,k\eda] $.
%		\State $V' \as \prod_{j=1}^{k} V_{i_j}^{-1}$ mod $n$
%		\State $\beta = \RSAEval(\gamma) \cdot V'$ mod $n$
%		\State If $H_1(\beta) = h$ then return 1, else return 0.
%	\end{algorithmic}
%\end{algorithm}

%Here, we prove the correctness!


%
%\begin{algorithm}[h]
%	\caption{Fast Authentication with Homomorphic One-Way functions (\fahow) - Compact Knapsack instantiation (\fahowCK)}\label{alg:FAHOW_CK}
%	\hspace{5pt}
%	\begin{algorithmic}[1]
%		\Statex   $\underline{(\sk,\pk)\as \fahowCKkg(1^{\kappa})}$: Executed offline (once).
%		\vspace{3pt}
%		\State $(t,k)$ are \hors~parameters as in Definition \ref{def-HORS}, and  $z\as\zo^{\kappa}$.
%		\State $(n,m,p)$ are \em Compact Knapsack \em parameters as in Definition \ref{def-compact}.
%		\State $s_i\as \PRF{i}$, $i = 1,\ldots,t$.
%		\State $V_i = F(s_i)$, $i = 1,\ldots,t$, where $ F_a $ is a \em compact knapsack \em function.
%		\State $\sk = (z,t,k,n,m,p)$, $\pk = (V_1,\ldots,V_t, t, k,n,m,p)$.
%	\end{algorithmic}
%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex $\underline{\sigma\as \fahowCKsig(m,\sk)}$: Given a message $m\in \zo^{*}$, compute its signature as follows:
%		\vspace{3pt}
%		\State $r \as \PRF{c}$, $R \as F_a(r)$, where $c$ is a counter starting from $t+1$.
%		\State $h \as H(R)$
%		\State $(i_1,\ldots,i_k) \as H(m||h)$, where $\{i_j\}_{j=1}^{k} \in [1,t]$.
%		\State $s_{i_j} \as \PRF{i_j}$, $j = 1,\ldots,k$.
%		\State $\gamma = (\sum_{j=1}^{k} s_{i_j}) + r$ mod $p$
%		\State $\sigma=(\gamma,h)$.
%	\end{algorithmic}
%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex $\underline{\zo\as \fahowCKver(m,\sigma,\pk)}$: Given $m\in \zo^{*}$, verify its signature $\sigma=(s,a)$ under $\pk=(Y,\beta)$ as follows:
%		\vspace{3pt}
%		\State $(i_1,\ldots,i_k) \as H(m||h)$
%		\State $V' \as \sum_{j=1}^{k} V_{i_j}$ mod $p$
%		\State $\beta = F_a(\gamma) - V'$ mod $p$
%		\State If $H(\beta) = h$ then return 1, else return 0.
%	\end{algorithmic}
%\end{algorithm}
%









==> ARIS Arxiv/Security.tex <==
\section{Security Analysis}\label{sec:security}
 We prove that \eda~is EU-CMA secure,  as defined in Definition \ref{def-EUCMA}, in the Random Oracle Model (ROM) \cite{Bellare:1993}. The proof   uses the Forking Lemma \cite{Bellare-Neven:2006}. 
 
 \begin{theorem}
In the ROM, if  adversary \A can  $(q_S,q_H) $-break the EU-CMA  security of  \eda~after making $ q_H $ and $ q_S $ random oracles and signature queries, respectively; then we can build another algorithm \B~that runs \A as a subroutine and can solve an instance of the ECDLP (as in Definition \ref{def:ECDLP}).
 \end{theorem}

\begin{proof}
We let $ Y^*\Ra \EC $  be an instance the  ECDLP  for algorithm \B~to solve. On the input of $ Y^* $ and $ z\Ra \Zp $, \B~works as follows. 

\noindent\underline{\emph{Setup:}} \B~keeps three lists $ \mathcal{L}_i $ for $ i\in\{1,2,3\} $ to keep track of the outputs of the random oracles and a list  $ \mathcal{L}_m $ to store the messages submitted to the sign oracle. \B~sets up the random oracle $RO$-$Sim(\cdot) $ to handle the hash functions and generates the users' public keys as follows.
\begin{itemize}
 \item \emph{Setup} $RO$-$Sim(\cdot)$: \B~implements $RO$-$Sim(\cdot) $ to handle queries  to hash functions $ \hash_1,\hash_2 $ and $ \hash_3 $, which are modeled as random oracles, as follows. 
 
 \begin{enumerate}
 	\item  $ \alpha_1 \gets  RO$-$Sim(m,z, \mathcal{L}_1)$: If $(m,z) \in   \LL_1$, it returns the corresponding value $ \alpha_1 $. Else, it returns $ \alpha_1 \Ra \{0,1\}^{l_1} $ as the answer and adds $  (m,z,\alpha_1) $ to $ \LL_1 $.
 	 	\item  $ \alpha_2 \gets  RO$-$Sim(R, \mathcal{L}_2)$: If $ R \in   \LL_2$, it returns the corresponding value $ \alpha_2 $. Else, it returns $ \alpha_2 \Ra \{0,1\}^{l_2} $ as the answer and adds $  (R,\alpha_2) $ to $ \LL_2 $.
 	  	 	\item  $ \alpha_3\gets  RO$-$Sim(m,h, \mathcal{L}_3)$: If $ (m,h) \in   \LL_3$, it returns the corresponding value $ \alpha_3 $. Else, it returns $ \alpha_3\Ra \{0,1\}^{l_1} $ as the answer and adds $  (m,h,\alpha_3) $ to $ \LL_3 $.	
 	 
 \end{enumerate}
 \item \emph{Setup Public Key}: Given the parameters $ (p,q,P,t,k) $, \B~works as follows to generate the user public key. 
  \begin{enumerate}
 	\item  Select $ j\Ra [1,t]$ and sets the challenge public key element $ Y_j \gets Y^* $.
 	\item Generate $ x_i \Ra  \Zp $ for $ i\in \{1,\dots,t\} $ and $ i\neq j $. 
 	\item Compute $ Y_i \gets x_i P $ for $ i\in \{1,\dots,t\} $ and $ i\neq j $.
 	\item Set $ \sk \gets \{x_i\}_{i=1,i\neq j} ^t $ and $ \pk \gets \{Y_1,\dots,Y_t\}$.
 	
 \end{enumerate}
\end{itemize}

\noindent\underline{$ \mathcal{A} $\emph{'s Queries:}} \A queries the hash functions $ \hash_i $ for $ i\in\{1,2,3\} $ and the sign oracle   for up to $ q_H $ and $ q_S $ times, respectively. \B~works as follows to handle these queries. 
\begin{itemize}
  \item \emph{Hash Queries:} $ \mathcal{A}$'s queries to hash functions $ \hash_1,\hash_2 $ and $ \hash_3 $ are handled by the $RO$-$Sim(\cdot) $ function described above.
  \item \emph{Signature Queries:}  \B~works as follows to answer $ \mathcal{A}$'s  signature query on message $ m $. If $ m\in \LL_m $, \B~retrieves the corresponding signature from $ \LL_m  $ and returns to $ \mathcal{A}$. Else, if $ m\notin \LL_m $, it works as follows.  

 \begin{enumerate}
	\item   Select $ s\Ra \Zp$ and compute $ S\gets sP $.
	\item Select $ k $   indexes $ (i_1,\dots i_k) \Ra [1,\dots,t]$.
 	\item  Set $ R  \gets  S - \sum_{i=1}^{k}Y_i$ and $ \alpha_2 \gets \{0,1\}^{l_2} $ and add $ (R,\alpha_2)  $ to $ \LL_2 $.
 	\item  If $  (\langle i_1,\dots i_k\rangle,h) \in \LL_3 $ abort. Else, add $  (m,h,\langle i_1,\dots i_k\rangle) $ to $ \LL_3 $. 
 	\item  Output $ \sigma =(s,h) $ to $ \mathcal{A}$ and add  $ (m,\sigma)\in\LL_m $.
\end{enumerate}




\end{itemize}
    \noindent\underline{$ \mathcal{A} $\emph{'s Forgery:}} Eventually, \A outputs a forgery  $ \sigma^* =(s^*,h^*) $ on message $ m^* $ and public key $ pk  $. Following the EU-CMA definition (as in Definition \ref{def-EUCMA}), \A only wins the game if $ \edaver(m^*,\sigma^*,pk) $ returns $ valid $ and $ m^* $ was never submitted to signature queries in the previous stage (i.e., $ m^*\notin \LL_m $).
    
\noindent\underline{\emph{Solving the ECDLP:}}  If \A does not output a valid forgery before making $ q_H $ hash queries and $ q_S $ signature queries, \B~also fails to solve the instance of ECDLP. Otherwise, if \A outputs a valid forgery    $ ( m^*,\sigma^* =\langle s^*,h^*\rangle ) $, using the forking lemma, \B~rewinds \A with the same random tape as in \cite{Bellare-Neven:2006}, to get a second forgery $  ( m',\sigma' =\langle s',h'\rangle ) $ where, with an overwhelming probability  $ s^* \neq s'  $ and $ h^*  = h' $. Based on  \cite[Lemma 1]{Bellare-Neven:2006}, $ \hash_3(m^*,h^*) \neq \hash_3(m^*,h') $, therefore, given $ (m^*,h^*) \in \LL_3$ and $ (m^*,h') \in \LL_3$,  \B~can solve a random instance of the ECDLP problem (i.e., $ Y^* $) if one of the following conditions hold. 
 \begin{itemize}
\item \textbf{Case 1:} For   $(i^*_1,\dots,i^*_k)  \gets \hash_3(m^*,h^*) $  and  $(i'_1,\dots,i'_k) \gets  \hash_3(m^*,h')    $   we have $ j\in (i^*_1,\dots,i^*_k) $ and $ j\notin (i'_1,\dots,i'_k) $.
\item  \textbf{Case 2:} For   $(i^*_1,\dots,i^*_k)  \gets \hash_3(m^*,h^*) $  and  $(i'_1,\dots,i'_k) \gets  \hash_3(m^*,h')    $   we have $ j\notin (i^*_1,\dots,i^*_k) $ and $ j\in (i'_1,\dots,i'_k) $.
\end{itemize}
If any of the above cases holds, \B~works as follows. If Case 1 holds, $ x_j \gets s^* -\sum_{\eta=1,\eta\neq j}^{k} x_{i^*_\eta}-s'-\sum_{\eta=1}^{k} x_{i'_\eta}\mod p$. Else, if Case 2 hold, $ x_j \gets s' -\sum_{\eta=1,\eta\neq j}^{k} x_{i'_\eta}-s^*-\sum_{\eta=1}^{k} x_{i^*_\eta}\mod p$. \end{proof}

==> ARIS Arxiv/commands.tex <==
\usepackage[para]{threeparttable}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{varwidth}
\newcommand{\Note}[1]{\textcolor{red}{#1}}
\usepackage{subcaption}
%ex
\setlength\floatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\textfloatsep{1.25\baselineskip plus 3pt minus 2pt}
\setlength\intextsep{1.25\baselineskip plus 3pt minus 2 pt}
\renewcommand\topfraction{0.85}
\renewcommand\bottomfraction{0.85}
\renewcommand\textfraction{0.1}
\renewcommand\floatpagefraction{0.85}
%  \usepackage{hyperref}  % hyperlinks\texttt{PRF}
%\usepackage[tight,footnotesize]{subfigure}
%\usepackage{url}
\usepackage{graphicx}
%\usepackage{theorem}
\usepackage{amsthm}

\usepackage[noend]{algpseudocode}
%\usepackage[noend]{algcompatible}
\usepackage{algorithm}

\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}

%\usepackage{float}% http://ctan.org/pkg/float
%\floatstyle{boxed} % Box...
%\restylefloat{figure}% ...figure environment contents.


\newenvironment{scheme}[2]
{\algorithm[#2] \renewcommand{\thealgorithm}{#1} }
{\endalgorithm}

\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}

\usepackage{tikz}
\usetikzlibrary{plotmarks}
\usepackage{pgfplots}
\usetikzlibrary{backgrounds}
\usetikzlibrary{patterns}
\usepgfplotslibrary{units}

\usepackage{epsfig}
\usepackage{url}
\usepackage{stfloats}
\usepackage{enumerate}
\usepackage{longtable}

%\usepackage[noend]{algorithmic}
%\usepackage{algpseudocode}

%\usepackage{pdfsync} %for synchronization with sumatrapdf
%\usepackage{caption}
%\usepackage{subfigure}
%\usepackage{url}
\usepackage{multirow}
%\usepackage{enumerate}
%\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{verbatim}
%\usepackage{amsmath}
\usepackage{amssymb}

%\usepackage{stfloats}
\usepackage{xspace}

\usepackage{xcolor}      % Used to highlight comments
%\usepackage[T1]{fontenc}
%\usepackage{microtype} % improves font spacing, needs pdfTEX >= 1.20

\newcommand{\NOTE}[1]{\textcolor{red}{#1}}
%% ENABLE THESE TWO LATER
%\usepackage{hyperref}  % hyperlinks
%\usepackage{subcaption} 




% Fonts
%\renewcommand{\rmdefault}{put} % Utopia
%\renewcommand{\sfdefault}{phv} % Helvetica
%\renewcommand{\ttdefault}{pcr} % Courier
%
% custom commands
\newcommand{\rpl}[1]{\textcolor{red}{#1}}
\newcommand{\draft}[1]{\textcolor{blue}{#1}}
\newcommand{\ctm}{\rpl{\textsuperscript{[citation missing}}}
\newcommand{\stl}{\rpl{\textsuperscript{[style incorrect]}}}
\newcommand{\cpm}{\rpl{\textsuperscript{[caption missing]}}}


% Abbreviations
\newcommand{\etal}{et~al.\@\xspace}
\newcommand{\etaltild}{et~al.\@~}
\newcommand{\eg}{e.g.,\@\xspace}
\newcommand{\ie}{i.e.,\@\xspace}
\newcommand{\ieenv}{isolated execution environment\@\xspace}

% Units
\newcommand{\MHz}{ MHz\xspace}
\newcommand{\GHz}{ GHz\xspace}
\newcommand{\mhz}{ MHz\xspace}
\newcommand{\kbyte}{K byte\@\xspace}
\newcommand{\kbytes}{K bytes\@\xspace}
\newcommand{\kbps}{ kbps\@\xspace}

% Misc.
\newcommand{\eat}[1]{}                % Comment out large swaths of text
\def \R { \overset{R}{\leftarrow} }   % Choose at random
\newcommand{\xor}{\oplus}             % Correct the omission of xor
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil }    % Ceiling function with proper sizing
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor } % Floor function with proper sizing
\newcommand{\rpick}{{\buildrel R \over \leftarrow}}
\newcommand{\eeq}{\mathrel{{:}{:}{=}}}
\newcommand{\X}{{\cal X}}
\newcommand{\qeq}{{\buildrel ? \over =}}
\newcommand{\zo}{{\{0,1\}}}

% Crypto Operations

\newcommand{\KDF}[2]{\ensuremath{\textrm{KDF}_{#1}\mskip-1mu(#2)}}
\newcommand{\Hash}[1]{H\mskip1mu(#1)}
\newcommand{\MAC}[2]{\textrm{MAC}_{#1}\mskip-1mu(#2)}

\newcommand{\kf}{\ensuremath{k_1}} % key used to encryp files
\newcommand{\kt}{\ensuremath{k_2}} % key used for trapdoor deviration
\newcommand{\kd}{\ensuremath{k_3}} % key used for key derivation
\newcommand{\F}[2]{\ensuremath{F_{#1}\mskip1mu(#2)}}
\newcommand{\G}[2]{\ensuremath{G_{#1}\mskip1mu(#2)}}
\newcommand{\HH}[1]{\ensuremath{H\mskip-1mu(#1)}}


\newcommand{\leakS}{\ensuremath{\mathcal{L}_1(\delta,\fb)}}
\newcommand{\leakA}{\ensuremath{\mathcal{L}_2(\delta,\fb,w,t)}}
\newcommand{\lS}{\ensuremath{\mathcal{L}_1}}
\newcommand{\lA}{\ensuremath{\mathcal{L}_2}}
\newcommand{\Real}{\ensuremath{\mathbf{Real}_{\mathcal{A}}(\kappa)}}
\newcommand{\Ideal}{\ensuremath{\mathbf{Ideal}_{\mathcal{A},\mathcal{S}}(\kappa)}}



\newcommand{\I}{\ensuremath{\mathbf{I}}}
\newcommand{\Ip}{\ensuremath{\mathbf{I}'}}
\newcommand{\II}{\ensuremath{\overline{I}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\II}{\ensuremath{\overrightarrow{I}}}


\newcommand{\V}{\ensuremath{V}}
\newcommand{\VV}{\ensuremath{\overrightarrow{V}}}
\newcommand{\U}{\ensuremath{U}}
\newcommand{\UU}{\ensuremath{\overrightarrow{U}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}


\newcommand{\TW}{\ensuremath{T_w}}
\newcommand{\TF}{\ensuremath{T_f}}
\newcommand{\Inf}{\ensuremath{\textrm{Inf}_u}}

\newcommand{\jj}{\ensuremath{y_j}}
\newcommand{\ii}{\ensuremath{i}}
\newcommand{\rr}{\ensuremath{r}}
\newcommand{\pad}{\ensuremath{pad}}
\newcommand{\st}{\ensuremath{\mathsf{st}}}
\newcommand{\GC}{\ensuremath{gc}}
\newcommand{\rb}{\ensuremath{\overline{r}}}
%\newcommand{\tb}[1]{\ensuremath{\tau'_{#1}}}
%\newcommand{\tf}{\ensuremath{\bf{\tau'_f}}}


\newcommand{\sw}{\ensuremath{s_w}}
\renewcommand{\sf}{\ensuremath{s_{id}}}

\newcommand{\tfp}{\ensuremath{s_{{id}_j}}}

\newcommand{\twp}{\ensuremath{s_{w_i}}}

\newcommand{\tf}{\ensuremath{\tau_f}}
\newcommand{\tfpp}{\ensuremath{\tau'_{f}}}
%
\newcommand{\tw}{\ensuremath{\tau_w}}
%\newcommand{\twp}{\ensuremath{\tau_{w_i}'}}
\newcommand{\ctb}{\ensuremath{\overline{\ct}}}

\newcommand{\blockct}{\ensuremath{u}}

\newcommand{\ct}{\ensuremath{u}}

\newcommand{\ctht}{\ensuremath{\mathsf{ct}}}
\newcommand{\idx}{\ensuremath{\mathsf{idx}}}

\newcommand{\idw}{\ensuremath{\mathcal{I}_{w}}}
\newcommand{\id}{\ensuremath{\mathcal{I}}}

\newcommand{\y}{\ensuremath{y}}
\newcommand{\yp}{\y'}

\newcommand{\x}{\ensuremath{x}}
\newcommand{\xp}{\x'}


\newcommand{\vect}[1]{\ensuremath{{\bf{#1}}}}

\newcommand{\m}{\ensuremath {m}{\xspace}}
\newcommand{\n}{\ensuremath {n}{\xspace}}
\newcommand{\f}{\ensuremath {f}}
\newcommand{\w}{\ensuremath {w}}

\newcommand{\fu}{\ensuremath {u}}
\newcommand{\du}{\ensuremath {d}}

\newcommand{\wb}{\ensuremath{\mathcal{W}}{\xspace}}

\newcommand{\fb}{\ensuremath {\mathcal{F}}{\xspace}}

\newcommand{\ci}{\ensuremath {c}{\xspace}} %ciphertext
\newcommand{\cib}{\ensuremath {\mathcal{C}}{\xspace}}

\newcommand{\Encr}[2]{\{#1\}_{#2}}
\newcommand{\Enc}[2]{\ensuremath{\mathcal{E}.\mathsf{Enc}_{#1}\mskip-1mu(#2)}}
\newcommand{\Dec}[2]{\ensuremath{\mathcal{E}.\mathsf{Dec}_{#1}\mskip-1mu(#2)}}
\newcommand{\Kg}[1]{\ensuremath{\mathcal{E}.\mathsf{Gen}\mskip-1mu(#1)}}

\newcommand{\FCSpace}{\ensuremath{(4\cdot\kappa)O(n\cdot m)+(2\cdot z)O(m)}}
\newcommand{\FCUpdComm}{\ensuremath{(2\cdot z\cdot \kappa)O(n\cdot \log_{2}(m))}}
\newcommand{\FCSearchtime}{\ensuremath{O(\frac{r}{p}\cdot log_2(m))}}
\newcommand{\FCUpdtime}{\ensuremath{O(\frac{2n}{p}\cdot log_2(m))}}

\newcommand{\SedghiUpdComm}{\ensuremath{O(n'\cdot m)}}

\newcommand{\CCSDSSESearchtime}{\ensuremath{O(r)}}



\newcommand{\OurSpace}{\ensuremath{O(n\cdot m)+\kappa\cdot O(m)}}
\newcommand{\OurUpdComm}{\ensuremath{O(n)}}
\newcommand{\OurSearchtime}{\ensuremath{\BigO{\frac{\NumOfFiles}{p}}}}
\newcommand{\OurUpdtime}{\ensuremath{\BigO(\frac{2n}{p})}}



%\mathsf{EKg}\mskip-1mu(#1)
\newcommand{\hi}{\ensuremath {\mathcal{HI}}{\xspace}}
\newcommand{\lh}{\ensuremath {\mathcal{LH}}{\xspace}}
\newcommand{\lk}{\ensuremath {\mathcal{LK}}{\xspace}}
\newcommand{\lr}{\ensuremath {\mathcal{LR}}{\xspace}}

\newcommand{\A}{$\mathcal{A}$~}
\newcommand{\Sim}{$\mathcal{S}$~}
\newcommand{\Q}{\textrm{Query}}
\newcommand{\SP}{\ensuremath{\mathcal{P}(\delta,\Q,t)}}
\newcommand{\AP}{\ensuremath{\Delta(\delta,\fb,w,t)}}
\newcommand{\ro}{\ensuremath {\mathit{RO}(\cdot)}{\xspace}}
\newcommand{\hsim}[1]{\ensuremath {\mathit{RO}\mskip1mu(#1)}}


\newcommand{\SSEEnc}{\ensuremath{\mathsf{Enc}}}
\newcommand{\SSEDec}{\ensuremath{\mathsf{Dec}}}
\newcommand{\Gen}{\ensuremath{\mathsf{Setup}}}
\newcommand{\SrchToken}{\ensuremath{\mathsf{SearchToken}}}
\newcommand{\Search}{\ensuremath{\mathsf{Search}}}
\newcommand{\AddToken}{\ensuremath{\mathsf{AddToken}}}
\newcommand{\Add}{\ensuremath{\mathsf{Add}}}
\newcommand{\DeleteToken}{\ensuremath{\mathsf{DeleteToken}}}
\newcommand{\Delete}{\ensuremath{\mathsf{Delete}}}




\newcommand{\MainSSEEnc}{\ourdsse.\ensuremath{\mathsf{Enc}}}
\newcommand{\MainSSEDec}{\ourdsse.\ensuremath{\mathsf{Dec}}}
\newcommand{\MainGen}{\ourdsse.\ensuremath{\mathsf{Setup}}}
\newcommand{\MainSrchToken}{\ourdsse.\ensuremath{\mathsf{SearchToken}}}
\newcommand{\MainSearch}{\ourdsse.\ensuremath{\mathsf{Search}}}
\newcommand{\MainAddToken}{\ourdsse.\ensuremath{\mathsf{AddToken}}}
\newcommand{\MainAdd}{\ourdsse.\ensuremath{\mathsf{Add}}}
\newcommand{\MainDeleteToken}{\ourdsse.\ensuremath{\mathsf{DeleteToken}}}
\newcommand{\MainDelete}{\ourdsse.\ensuremath{\mathsf{Delete}}}
\newcommand{\MainUpdateToken}{\ourdsse.\ensuremath{\mathsf{UpdateToken}}}
\newcommand{\MainUpdate}{\ourdsse.\ensuremath{\mathsf{Update}}}

\newcommand{\Update}{\ensuremath{\mathsf{Update}}}
\newcommand{\set}[1]{\mathcal{#1}}

% Protocol Tools
\newcommand{\Send}[3]{{#1}\rightarrow{#2}:&{#3}}
\newcommand{\Msg}[1]{\langle{#1}\rangle}

\newcounter{linecounter}
\newcommand{\resetlinecounter}{\setcounter{linecounter}{1}}
\newcommand{\llabel}[1]{\arabic{linecounter}. \addtocounter{linecounter}{-1}\refstepcounter{linecounter}\label{#1}\stepcounter{linecounter}}
\newcommand{\declabel}{\addtocounter{linecounter}{-1}}

\newcommand{\aboveleftarrow}[1]{{\buildrel #1 \over \longleftarrow}}
\newcommand{\aboverightarrow}[1]{{\buildrel #1 \over \longrightarrow}}
\newcommand{\aboveleftrightarrow}[1]{{\buildrel #1 \over \leftrightarrow}}


\newcommand{\vm}{\ensuremath {\overrightarrow{m}}{\xspace}}
\newcommand{\vM}{\ensuremath {\overrightarrow{M}}{\xspace}}
\newcommand{\ms}{\ensuremath {m^{\ast}}{\xspace}}


\newcommand{\hh}{\ensuremath {\overline{h}}{\xspace}}
\newcommand{\vv}{\ensuremath {\overline{v}}{\xspace}}

\newcommand{\Ra}{\ensuremath {\stackrel{\$}{\leftarrow}{\xspace}}}
\newcommand{\as}{\ensuremath {\leftarrow}{\xspace}}

\newcommand{\NumOfFiles}{\ensuremath{{n}}}
\newcommand{\NumOfWords}{\ensuremath{{m}}}
\newcommand{\NumOfActualKwFilePair}{\ensuremath{N'}}
\newcommand{\NumOfBlocks}{\ensuremath{{D}}}
\newcommand{\blocksize}{\ensuremath{b}}
\newcommand\myedit[1]{\textcolor{blue}{(#1)}}

\newcommand{\ourdsse}{\textsf{FS-DSSE}}
\newcommand{\ourdsselink}{\url{https://github.com/thanghoang/IM-DSSE/}}
\newcommand{\main}{\ourdsse^{\ensuremath{\mathsf{main}}}}
\newcommand{\variantI}{\ourdsse\textsuperscript{\textsf{I}}}
\newcommand{\variantII}{\ourdsse\textsuperscript{\textsf{II}}}
\newcommand{\variantIII}{\ourdsse\textsuperscript{\textsf{I+II}}}

\newcommand{\mainshort}{\textsf{main}}
\newcommand{\varI}{\textsf{I}}
\newcommand{\varII}{\textsf{II}}
\newcommand{\varIII}{\textsf{I+II}}

% Thang command

\newcommand{\BigO}[1]{\ensuremath{\mathcal{O}\mskip1mu\left(#1\right)}}


\newcommand{\numoffiles}{\ensuremath{M}}

\newcommand{\seu}{\ensuremath{SEU-DSSE}}

%\theoremstyle{remark}
\newtheorem{remark}{Remark}

%\usepackage[hang,flushmargin]{footmisc}

\usepackage{enumitem}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\textcolor{green}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

\newcommand{\No}{\xmark}
\newcommand{\Yes}{\cmark}

	\newcommand{\sk}{\ensuremath {\mathit{sk}}{\xspace}}
\newcommand{\pk}{\ensuremath {\mathit{pk}}{\xspace}}



\newcommand{\RSAGen}{\ensuremath{\texttt{Gen}_{\texttt{RSA}}{\xspace}}}


\newcommand{\RSASamp}{\ensuremath{\texttt{Samp}_{\texttt{RSA}}{\xspace}}}

\newcommand{\RSAEval}{\ensuremath{\texttt{Eval}_{\texttt{RSA}}{\xspace}}}

\newcommand{\RSAInvert}{\ensuremath{\texttt{Invert}_{\texttt{RSA}}{\xspace}}}


\newcommand{\eda}{\ensuremath {\texttt{\textbf{ARIS}}}{\xspace}}
\newcommand{\edaRsa}{\ensuremath {\texttt{\textbf{ARIS}.RSA}}{\xspace}}
\newcommand{\edakg}{\ensuremath {\texttt{\textbf{ARIS}.Kg}}{\xspace}}
\newcommand{\edasig}{\ensuremath {\texttt{\textbf{ARIS}.Sig}}{\xspace}}
\newcommand{\edaver}{\ensuremath {\texttt{\textbf{ARIS}.Ver}}{\xspace}}

\newcommand{\edaCK}{\ensuremath {\texttt{CEDA{-}CK}}{\xspace}}
\newcommand{\edaCKkg}{\ensuremath {\texttt{CEDA{-}CK.Kg}}{\xspace}}
\newcommand{\edaCKsig}{\ensuremath {\texttt{CEDA{-}CK.Sig}}{\xspace}}
\newcommand{\edaCKver}{\ensuremath {\texttt{CEDA{-}CK.Ver}}{\xspace}}


\newcommand{\Fq}{\ensuremath {\mathbb{F}_q}{\xspace}}
\newcommand{\EC}{\ensuremath {E(\Fq) }{\xspace}}
\newcommand{\Zp}{\ensuremath {\mathbb{Z}_p}{\xspace}}
\newcommand{\prf}{\ensuremath {\texttt{PRF}}{\xspace}}
\newcommand{\hash}{\ensuremath {\texttt{H}}{\xspace}}
 \newcommand{\B}{\ensuremath{\mathcal{B}}{\xspace}}
 \newcommand{\RO}{\ensuremath {\texttt{RO}}{\xspace}}
 
 
  \newcommand{\LL}{\ensuremath{\mathcal{L}}{\xspace}}

==> ARIS Arxiv/conclusion.tex <==
\section{Conclusion}\label{sec:Conclusion}
In this paper, we presented a new efficient signature scheme to meet the strict minimum  delay requirements of  some real-time IoT systems.  This is achieved by harnessing the homomorphic property of the underlying ECDLP-based one-way function  and the precomputation technique proposed in \cite{BPV:basepaper:1998}. Our experimental results showed that the proposed scheme outperforms its state-of-the-art counterparts in signing and verification speed  as well as in energy efficiency.  The proposed scheme is shown to be secure, in the Random Oracle Model, under the hardness of the ECDLP. We   open-sourced our implementation  to enable public testing and verification. 
\vspace{1mm}

\noindent \textbf{Acknowledgment. }  This work is supported by  the Department of Energy award DE-OE0000780 and NSF award  \#1652389.

 

==> ARIS Arxiv/introduction.tex <==
\section{Introduction}\label{sec:Introduction}

 IoT systems often need authentication  for applications that need to verify  a large volume of incoming transactions or commands. While   symmetric key primitives (e.g., HMAC) can provide very fast authentication, they fail to offer non-repudiation which is often vital for these applications. For instance, Visa handles   millions of transactions every day \cite{VisaCard}.  Each transaction corresponds to multiple authentications of the user's request and card information on merchant's side, payment gateway and credit card issuer \cite{CreditCardinfra}.  Therefore,  creating more efficient solutions can significantly reduce the overall authentication overhead of such systems that results in substantial financial gains. 
 
The need for efficient authentication becomes even more imperative for applications in which IoT devices must operate in safety-critical settings and/or with battery limitations. For instance, battery-powered aerial drones \cite{Drone:Elisa:Won:2015} might communicate and authenticate streams of commands and measurements with an operation center in  a short period of time. A fast and energy-efficient authentication can improve the flight and response time of such aerial drones \cite{Dronecrypt}. Other IoT applications such as smart grid  systems, which involve battery-powered sensors, will also  benefit from fast and energy-efficient digital signatures  which minimize the   authentication delay/overhead and improve the operation time of  the  sensors~\cite{SmartGrid:PMU:Experiment:Journal:2017}.
Additionally,  in vehicular networks, safety significantly hinges  on the  end-to-end delay~\cite{IEEE1609.2_SecServices}, and therefore attaining  a signature scheme with the lowest end-to-end delay is always desired. 
 
 
% Additionally,  in vehicular networks, the lower end-to-end delay corresponds to the faster response time which safety significantly hinges  on the  end-to-end delay~\cite{IEEE1609.2_SecServices}, and therefore   need highly fast digital signatures for their safe and scalable operations.
\subsection{Our Contributions}

In this paper, we propose a new efficient signature scheme called \eda.  
%The main idea behind \eda~(as further elaborated in \Cref{sec:proposed}) is to leverage the  product of power property of exponents to efficiently  obtain polynomially-bounded multiple time signature schemes.  
\eda~makes use of an Elliptic Curve Discrete Logarithm Problem (ECDLP) based  one-way  function   and exploits the homomorphic properties of such functions to (i) linearly add the private key elements to attain a shorter signature and (ii) mask this addition with a one-time randomness $ r $ to achieve a (polynomially-bounded) multiple-time signature scheme.  
We outline the main properties of \eda~as below. 
\begin{itemize}
 

%\noindent$\bullet$\underline{  \em Fast Verification:} 
\item \underline{\em Fast Verification:} 
\eda~provides the fastest signature verification among its counterparts. More specifically, \eda~pushes the limits of   elliptic curve (EC) based signature schemes by providing  nearly $ 2\times  $ faster verification as compared to its fastest counterpart \cite{SchnorrQ}.  %This translates to the verification ability of 83,333 signatures per second on commodity hardware.  





%\noindent$\bullet$\underline{  \em Fast Signing:} 
\item \underline{\em Fast Signing:}  The signature generation of \eda~avoids  expensive computations such as  fixed-base scalar multiplication. Therefore, \eda~achieves 33\% faster signing as compared to its fastest counterpart \cite{SchnorrQ}. 

%\noindent$\bullet$\underline{  \em Low End-to-End Delay:} 
\item \underline{\em Low End-to-End Delay:} 
Due to having the fastest signature generation and  verification algorithms, \eda~achieves nearly $ 40\% $ lower end-to-end delay, as compared to its fastest counterpart \cite{SchnorrQ}.  This might encourage the potential  adoption of  \eda~for applications that require delay-aware authentication. 




%\noindent$\bullet$\underline{  \em Energy Efficiency:} 
\item \underline{\em Energy Efficiency:} 
 By avoiding any computationally expensive operation in the signing and verification algorithms, \eda~achieves the lowest energy consumption as compared to its state-of-the-art efficient counterparts.  Specifically,  as shown in Figure \ref{fig:sign}, the verification algorithm in \eda~attains $ 40\% $ lower energy consumption as compared to its most energy efficient counterpart. This makes \eda~potentially suitable for IoT applications wherein the battery-powered devices authenticate telemetry and commands (e.g., aerial drones).  


 

%\noindent$\bullet$\underline{  \em Tunable Parameters:}
\item \underline{\em Tunable Parameters:}  \eda~enjoys from a highly tunable set of parameters. This allows \eda~to be instantiated with different properties for different applications. For instance, the parameters set that we considered for our implementation on AVR microcontroller enjoys from a smaller public key and private key pair, and if the same scheme is implemented on commodity hardware, it can enjoy from a faster signature generation ($ 2\times $ faster than the scheme in \cite{SchnorrQ})  by incurring a few microseconds on the verification algorithm. 
\end{itemize}
\noindent\textbf{Limitations: } All of the desired properties and efficiency gains in \eda~come with the cost of  larger key sizes. For instance, in the verification efficient instantiation of \eda~(as in Table \ref{tab:Laptop}), which has the largest key sizes, the size of the public key and private key could be as large as $ 32$KB. However, this can be   decreased to  $  16$KB and $ 8 $KB for the private key and public key sizes (respectively) while still maintaining the fastest signature generation and verification algorithms among its counterparts.  We have shown that even with these parameters sizes, \eda~can be implemented on 8-bit AVR  while enjoying from the most computation and energy efficient algorithms as shown in  Figure \ref{fig:sign}, Figure \ref{fig:verify} and Table \ref{tab:AVR}.
 

\begin{figure*} 
	%\vspace{0mm}
	\centering
	\begin{minipage}[b]{.45\textwidth}
		\includegraphics[width=1\linewidth]{fig/fig-sign.pdf}
		\caption{Energy consumption (mJ) for signature generation of \eda~and its counterparts on AVR microcontroller}	\label{fig:sign}
		%\caption{\small{Our system model, where an authority (e.g., FAA, U.S. Department of Transportation) assigns self-certified AQ keys to the drones, and then ZSPs, control stations, drones etc. communicate over an insecure channel.}}
	\end{minipage}\qquad
	%\vspace{0mm}
	\begin{minipage}[b]{.45\textwidth}
		\includegraphics[width=1\linewidth]{fig/fig-verify.pdf}
		\caption{Energy consumption (mJ) for signature verification of  \eda~and its counterparts on AVR  microcontroller}	\label{fig:verify}
	\end{minipage}
	%\caption{\small{Our system model, where an authority (e.g., FAA, U.S. Department of Transportation) assigns self-certified AQ keys to the drones, and then ZSPs, control stations, drones etc. communicate over an insecure channel.}}
	
\end{figure*}

==> ARIS Arxiv/performance.tex <==
\section{Performance Evaluation}\label{sec:Performance}
 
We have fully implemented \eda~on Four$ Q $ curve \cite{FourQ} which is known to be the fastest EC that provides 128-bit of security. We provide   implementations of \eda~ on both  commodity hardware and 8-bit microcontroller to evaluate its performance since most IoT applications are comprised  of them both (e.g., commodity hardware as servers or control centers and microcontrollers as IoT devices connected to sensors).  We compare the performance of \eda~with state-of-the-art digital signature schemes on both of these platforms, in terms of computation, storage and communication. Our implementation is open-sourced at the following link.


\begin{center}
	\url{https://github.com/rbehnia/ARIS} 
\end{center}




%No analytical analysis.

%discuss fastness (especially in verification, we don't require double scalar multiplication) and energy also we can store keys in even 8-bit.

%9.891020us per sign
%12.995110us per verification
%Signing runs in ...................................... 25642 cycles
%Verify runs in ....................................... 33697 cycles
%22.886130us end-to-end delay

\subsection{Performance on Commodity Hardware}

\subsubsection{Hardware Configurations} We used a laptop equipped with Intel i7 Skylake processor @ $2.60$ GHz and $12$ GB RAM. 

\subsubsection{Software Libraries} We implemented \eda~using the open-sourced Four$ Q $ implementation~\cite{FourQ}, that offers the fastest EC operations, specifically EC additions that is critical for the performance of \eda. We used an Intel processor as our commodity hardware and leveraged Intel intrinsics to optimize our implementation. Specifically, we implemented our $\prf$ functions with Intel intrinsics (AES in counter mode). We used   blake2 as our hash function~\cite{blakeHash} due to its efficiency. 

We ran the open-source implementations of our counterparts on our hardware to compare their performance with \eda.

\subsubsection{Parameter Choice} Since we implement \eda~on Four$ Q $ curve, we use its parameters given in~\cite{FourQ}, which provide $128$-bit security. Other than the curve parameters, the choice of $t,k$ also plays a crucial role for the security of \eda. Specifically, $k$-out-of-$t$ combinations should also provide $128$-bit security to offer this level of security overall. On the other hand, we  can tune these parameters to achieve  our desired security level with different performance trade-offs. If we increase $t$ and decrease $k$, this results in a larger storage with faster computations,  and vice versa. For our commodity hardware implementation, we choose $t=1024$ and $k=18$, that we believe offers a reasonable trade-off between storage and computation as well as offering the desired $128$-bit security level. We set $ l_1 = 180 $ and $ l_2 =256 $.

\subsubsection{Experimental Results} We present the results of our experiments in Table \ref{tab:Laptop}. We observe that \eda~offers very fast signature generation and verification. It only takes 9 microseconds to generate a signature and 12 microseconds to verify it. This is the fastest among our counterparts, where the closest is SchnorrQ. Furthermore, if we use the same parameters set as for the AVR microcontroller, we can further speed up the signature generation to $ 6.5 $ microseconds, with the cost of a few microseconds on the verification speed. In SchnorrQ, a scalar multiplication is required in signature generation and a double scalar multiplication in verification. In \eda, EC additions are required for signature generation and verification is done with a scalar multiplication and EC additions. This corresponds to a $33\%$ faster signature generation and $83\%$ faster verification for \eda, compared to SchnorrQ. Therefore, we believe \eda~can be an ideal alternative for real-time applications.

\eda~signature size is the same with its EC-based counterparts \cite{ECDSA,Ed25519,Kummer,SchnorrQ} , that is significantly lower than its RSA-based and hash-based counterparts \cite{RSA,CEDA,SPHINCS}. On the other hand, \eda~comes with a larger private and public key, that is $32$ KB. 

\begin{table*}[t!]
	\centering
 	\vspace{ 2mm}


	\caption{Experimental performance comparison of \eda~and its counterparts on a commodity hardware} \label{tab:Laptop}
%	\vspace{-2mm}
	\begin{threeparttable}
		\begin{tabular}{| c || c | c | c | c |  c | c | }
			\hline
			\textbf{Scheme} & \specialcell[]{\textbf{Sign Generation}\\  \textbf{ Time (}$\mu$s\textbf{)}} & \specialcell[]{\textbf{Private Key}\textsuperscript{$ \dagger$} \\ \textbf{(KB)}} & \specialcell[]{\textbf{Signature }\\  \textbf{Size (KB)}} & \specialcell[]{\textbf{Signature Verification}\\  \textbf{ Time (}$\mu$s\textbf{)}} & \specialcell[]{\textbf{Public Key} \\ \textbf{(KB)}} & \specialcell[]{\textbf{End-to-End} \\ \textbf{Delay (}$\mu$s\textbf{)}} \\ \hline \hline 
			
			%			RSA & 11374.27 & 384 & 384 & 275.65 & 386 & 11649.92 \\ \hline
			
			SPHINCS~\cite{SPHINCS} & $13458$ & $1.06$ & $41000$ & $370$ & $1.03$ & $13828$\\ \hline
				TACHYON~\cite{Tachyon} & $138$ & $0.016$ & $4.4$ & $18$ & $864$ & $156$\\ \hline
			RSA~\cite{RSA}  & $8083$ & $0.75$ & $0.41$ & $48 $& $0.38$ & $8131$ \\ \hline 
			
			CEDA~\cite{CEDA}  & $55$ & $0.41$ & $0.41$ & $115$ & $384.38$ & $170$ \\ \hline 
			
			%			XMSS~\cite{} & $2^{\kappa}$& & & & & & \\ \hline 
			
			ECDSA~\cite{ECDSA}  & $725 $& $0.03$ & $0.06$ & $927$ & $0.03$ & $1652$\\ \hline
			
			Ed25519~\cite{Ed25519} &  $132$ &$ 0.03$ & $0.06$ & $335$ & $0.03$ & $467$ \\ \hline
			
			Kummer~\cite{Kummer} &  $23$ & $0.03$ & $0.06$ & $38$ & $0.03$ & $61$ \\ \hline 
			
			SchnorrQ~\cite{SchnorrQ} &  $12$ & $0.03$ & $0.06$ & $22$ & $0.03$ & $34$ \\ \hline \hline
			
			\eda  & $\mathbf{9}$ & $32.03$ & $0.06$ & $\mathbf{12}$ & $32$ & $\mathbf{21}$ \\ \hline 			
			
%			\multirow{3}{*}{\eda} & 1 & \multirow{3}{*}{\textbf{2 425}} & \multirow{3}{*}{\textbf{32}} & \multirow{3}{*}{\textbf{32}} & \multirow{3}{*}{52 872} & 96 & \multirow{3}{*}{\textbf{55 297}} \\ 
%			
%			& $2^{10}$&  &  & & & 64KB & \\ 
%			
%			& $2^{17}$&  &  & & & 8MB & \\ \hline
			
		\end{tabular}
		\begin{tablenotes}[flushleft]\scriptsize{  % switch locally to single-spacing
%				\item $\ddagger$ The sizes are in terms of \textbf{Bytes}, if otherwise not specified.
				
				\item $ \dagger $ System wide parameters (e.g., p,q,$\alpha$) for each scheme are included in their corresponding codes, and private key size denote to specific private key size.
				
%				\item The cost of hash-based schemes are estimated based on the cost of a single hash operation.
				
				%				\item The parameters for multiple-time signatures are selected such that they can sign XXX messages with a single key pair.
			}
		\end{tablenotes}
	\end{threeparttable}
	% }
%	\vspace{-3mm}
\end{table*}
\begin{table*} [t]
	\centering
	%\vspace{-2mm}
	\caption{Experimental performance comparison of \eda~and its counterparts on 8-bit AVR microcontroller} \label{tab:AVR}
	%	\vspace{-2mm}
	\begin{threeparttable}
		\begin{tabular}{| c || c | c | c | c |  c | c | }
			\hline
			\textbf{Scheme} & \specialcell[]{\textbf{Signature Generation}\\  \textbf{ Time (}s\textbf{)}} & \specialcell[]{\textbf{Private Key} \\ \textbf{(KB)}} & \specialcell[]{\textbf{Signature }\\  \textbf{Size (KB)}} & \specialcell[]{\textbf{Signature Verification}\\  \textbf{ Time (}s\textbf{)}} & \specialcell[]{\textbf{Public Key} \\ \textbf{(KB)}} & \specialcell[]{\textbf{End-to-End} \\ \textbf{Delay (}s\textbf{)}} \\ \hline \hline 
			
			
			%			SPHINCS~\cite{SPHINCS} & 2 681 600 389 & 1088 & 41000 & 16760.00  & 6115.56 \\ \hline 
			
			%			XMSS~\cite{} & $2^{\kappa}$ & & & & &  \\ \hline 
			
			ECDSA~\cite{ECDSA} & $1.77$ & $0.03$ & $0.06$  & $1.80$ & $0.03$ & $3.57$ \\ \hline
			
			Ed25519~\cite{Ed25519, Ed255198bit} & $1.45$ & $0.03$ & $0.06$  & $2.06$ & $0.03$ & $3.51$  \\ \hline 
			
			$\mu$Kummer~\cite{Kummer, Kummer8bit} &  $0.65$& $0.03$ & $0.06$  & $1.02$& $0.03$  & $1.67$  \\ \hline 
			
			SchnorrQ~\cite{SchnorrQ, FourQ8bit} & $0.27$& $0.03$ & $0.06$  & $0.60$& $0.03$  & $0.87$\\ \hline \hline
			
			\eda  & $\mathbf{0.19} $ & $16$ & $0.06$ & $\mathbf{0.37}$ & $8$ & $\mathbf{0.56}$ \\ \hline
			
		\end{tabular}
		\begin{tablenotes}[flushleft] \scriptsize{
				
			} % switch locally to single-spacing
			
		\end{tablenotes}
	\end{threeparttable}
	% }
	 \vspace{-4mm}
\end{table*}


\subsection{Performance on 8-bit AVR}

\subsubsection{Hardware Configurations} We used an 8-bit AVR ATmega 2560 microcontroller as our IoT device to implement \eda. ATmega 2560 is equipped with $256$ KB flash memory, $8$ KB SRAM and $4$ KB EEPROM, with a maximum clock frequency of $16$ MHz. ATmega 2560 is extensively used in practice for IoT applications (especially in medical implantables) due to its energy efficiency~\cite{ATmega2560Medical}.

\subsubsection{Software Libraries} We implemented \eda~on ATmega 2560 using the 8-bit AVR implementation of Four$ Q  $ curve~\cite{FourQ8bit}, that provides the basic EC operations and a blake2 hash function. We implemented our scheme with IAR embedded workbench and used its cycle-accurate simulator for our benchmarks. 

As for our counterparts, we used their open-sourced implementations~\cite{Ed255198bit,Kummer8bit,FourQ8bit,microECC}. Note that we only compare \eda~with its EC-based counterparts, due to their communication and storage efficiency. Moreover, resource-contrained processors such as ATmega 2560 may not be suitable for heavy computations (e.g., exponentiation with 3072-bit numbers in RSA \cite{RSA}  and CEDA \cite{CEDA}). 

\subsubsection{Parameter Choice} As mentioned, \eda~can be instantiated with different $t,k$ values that offers a trade-off between storage and computation. Since ATmega 2560 is a storage-limited device, we select our parameters as $ t = 256$ and $k = 28$ to offer storage efficiency. Moreover, this allows us to store the private components ($x_i$ and $r_i$), instead of deterministically generating them at signature generation, and still have a tolerable storage even for an 8-bit microcontroller.  We also set $ l_1 \gets 224 $ and $ l_2 \gets 256 $.

%Suggestion: Change Parameters to t = 256 and k = 28 and store the secret values (each 128-bit) as well instead of deterministically generating them, for better performance and storage here (for 8-bit)!




\subsubsection{Experimental Results} Table \ref{tab:AVR}~shows the performance of \eda~compared with its  counterparts. The speed improvements of \eda~can also be observed for ATmega 2560. \eda~is $42\%$ faster in signature generation and $76\%$ faster in signature verification compared to its closest counterpart \cite{SchnorrQ}. This can translate into a significant practical difference when considered real-time applications that require fast authentication. Note that these benchmarks are obtained with a more ``storage friendly'' parameter choice, and can be further accelerated with different parameter choices where the microcontroller  is not memory-constraint.

One may notice that due to our parameter choice, the key sizes in our 8-bit microcontroller implementation are smaller. As aforementioned, this is because we select a different parameter set for $t,k$. Moreover, we store the private components as well, that correspond the 8 KB of the signer storage. Since we store these keys on the flash memory of ATmega 2560, they only correspond to $6\%$ and $3\%$ of the total memory, for private key and public key, respectively. Therefore, although we have significantly larger keys than our EC-based counterparts, it is still feasible to store them even on highly resource-constrained 8-bit microcontrollers.

\subsubsection{Energy Efficiency} It is highly desirable to minimize the energy consumption of cryptographic primitives in IoT applications to offer a longer battery life. For microcontrollers, energy consumption of the device can be measured with the formula $E = V * I * t$, where $V$ is voltage, $I$ is current and $t$ is the computation time~\cite{Precomputation:LowCostSig:Ateniese:NDSS2013}. Considering that the voltage and the current of a microcontroller are constant when the device is active, the energy consumption linearly increases with the computation time. Since \eda~offers the fastest signature generation and verification, energy consumption of \eda~is the lowest among its counterparts, and therefore would be preferred in applications that require longer battery life.


%To sign, we need 36 PRFs, 3 hash, 1 BPV Online + additions mult etc.
%To calculate ARIS: BPV Online with k = 18 ----> 1303890 cycles
%To calculate ARIS: BPV Online with k = 28 ----> 1970130 cycles
%Blake 2b -----> 380033 cycles (output is 512 bits)
%if we used Rhys Weatherley -> 32000 cycles! (blake2s, with 256-bit output)
%ecc mul fixed ----> 2979848 cycles
%addition 171 x 56
%mult 5693
%ARIS SIGN = 3065498 cycles + 100.000 safety = 3165498
%ARIS VERIFY = 5810044 cycles + 100.000 safety = 5910044





==> ARIS Arxiv/preliminaries.tex <==

\section{Preliminaries}\label{sec:Prelim}


\noindent \textbf{Notation.} Given two primes $ p $ and $ q $ we define a finite field \Fq~and a group \Zp.  We also work on \EC~as an elliptic curve over   \Fq. We commonly denote $ P\in \EC $ as a generator of the points on the curve.  $ x\Ra S $ denotes randomly selecting      $ x  $ from a set $ S $. We denote scalars as small letters (e.g., $ x $) and points on curve as capital letters (e.g., $ P $).   We denote tables/matrices as bold capital letters (e.g., $ \mathbf{P} $). We define the bit-length of a variable  as $ |x| $, i.e., $ |x| = \log_2 x $. Scalar and point multiplication is denoted as $ xP $.  We define two Pseudo Random Functions 			$\texttt{PRF}_1: \{0,1\}^*\rightarrow \Zp$  and 	$\texttt{PRF}_2: \{0,1\}^*\rightarrow \{0,1\}^\kappa$  and three hash function $\hash_1:\{0,1\}^* \times \Zp \rightarrow \{0,1\}^{l_1}$, $\hash_2:\EC \rightarrow \{0,1\}^{l_2}$, and $\hash_3:\{0,1\}^* \times \{0,1\}^{l_2} \rightarrow \{0,1\}^{l_1}$  for some integers $ l_1 $ and $ l_2 $, to be defined in Section \ref{sec:Performance}.
%
%\begin{table}[h]
%	\centering
%	\vspace{-3mm}
%	\caption{Notation in $\ourdsse$ scheme.} \label{tab:Notation}
%	%		\resizebox{\textwidth}{!}{
%	%\footnotesize
%	%\vspace{-3mm}
%	\begin{threeparttable}
%		\begin{tabular}{| r | l |}
%			\hline
%			%			$\mathcal{E}$ & IND-CPA Encryption Scheme \\ \hline
%			%			$G_k$ & Pseudo Random Function (PRF) with Key k \\ \hline 
%			$\I$ & Incidence matrix-based encrypted index\\ \hline
%			%			$\delta$ & Unencrypted Incident Matrix \\ \hline
%			%$\y_j$ & Column (File) Index \\ \hline
%			%$\x_i$ & Row (Keyword) Index \\ \hline
%	%		$j$ & Column (File) Index \\ \hline
%	%		$i$ & Row (Keyword) Index \\ \hline
%			$w_i, f_j$ & Keyword and file with IDs $i$, $j $, resp. \\ \hline
%%			$\f_j$ & File indexing at column $ j $ in $ \I $ \\ \hline
%			$r_i$ & Row key \\ \hline
%			$u_i$ & Row counter (initially set to 1) \\ \hline
%			$v_i$ & Row state (0 if row key is revealed to server, 1 otherwise) \\ \hline
%			%			$v_j$ & Column Counter (Initially set to 1) \\ \hline
%			%			$s_{w_i}$ & Row (Keyword) Key Generated by $G_k$\\ \hline 			
%			$c$ & Encrypted file \\ \hline
%			$n, m$ & Maximum number of keywords and files in DB, resp. \\ \hline
%	%		$m$ & Maximum number of keywords \\ \hline
%			$D[i]$ & Dictionary to store file indexes for each keyword \\ \hline
%			$\TW$ & Keyword hash table \\ \hline
%	%		$\TW$ & Keyword hash table. \\ \hline
%	%		$\TF$ & File hash table \\ \hline
%			$\I[i,j].st$ & State bit indicating last access\textsuperscript{$ \dagger $} on $ \I[i,j] $ \\ \hline
%		\end{tabular}
%		\textsuperscript{$\dagger $}$ \I[i,j].st = 1 $ if last access is update, and $ \I[i,j].st = 0 $ if it is search.
%	\end{threeparttable}
%	\vspace{-3mm}
%\end{table}


\begin{definition} \label{def:ECDLP}\normalfont ({\em Elliptic Curve Discrete Logarithm Problem}) For \EC~as an elliptic curve over a finite field \Fq,  given  $ P,Q\in \EC  $,  the Elliptic Curve Discrete Log Problem (ECDLP) asks  to find $ k  \in \Zp$,  if  it exists, such that  $ Q=kP $.
 
\end{definition}






\begin{definition}\normalfont
	A  signature scheme consists of three algorithms $  \texttt{SGN} = (\texttt{Kg,Sig,Ver}) $ defined as follows.
	
	\begin{itemize}\normalfont
		\item[--] $ (\sk, \pk) \leftarrow \texttt{SGN.Kg}(1^\kappa) $: Given the security parameter $ \kappa $, it outputs the private and public key pair $ (\sk,\pk) $.
		
		\item[--] $ \sigma \leftarrow \texttt{SGN.Sig}(m,\sk) $:
		Given the message   $ m $ and the signer's private key  $\sk$, it outputs the signature $ \sigma $.
		\item[--] $ \{0,1\} \leftarrow \texttt{SGN.Ver}(m, \sigma, \pk) $: Given a message-signature pair   ($m,\sigma $), and the claimed signer's public key  $\pk$, it outputs a decision bit  $ d \gets \{0,1\} $.
	\end{itemize}
\end{definition}

In the following definition, we define the security of signature schemes based on the methodology proposed in \cite{Bellare-2006}.  After the initialization phase i.e., $ \texttt{SGN.Kg}(\cdot) $,  The adversary \A  is given access to the signature generation oracle. \A  wins, if it outputs a \emph{valid} message-signature pair (that was not previously outputted from the sign oracle)  after making polynomially-bounded number of queries. 

\begin{definition}\label{def-EUCMA}\normalfont
Existential Unforgeability under Chosen Message Attack (EU-CMA)  experiment $ \mathit{Expt}^{\mathit{EU-CMA}}_{\mathtt{SGN}} $   is defined as follows.
\begin{itemize}\normalfont
\item [--] $ (\sk,\pk)\leftarrow \texttt{SGN.Kg}(1^\kappa) $
\item[--] $ (m^*, \sigma^*)\leftarrow  \mathcal{A}^{\texttt{SGN.Sig}(\cdot)} (\pk) $
\item[--]  If $  1 \leftarrow {\texttt{SGN.Ver}(m^*, \sigma^*, \pk)} $ and $ m^* $ was not queried to $ \texttt{SGN.Sig}(\cdot) $, return 1, else, return 0.

\end{itemize}

The EMU-CMA advantage of    \A     is defined as $ \mathit{Adv}^{\textit{EU-CMA}}_{\texttt{SGN}} =  \Pr[ \mathit{Expt}^{\mathit{EU-CMA}}_{\texttt{SGN}}= 1]$.
\end{definition}


%\noindent \textbf{System Model.} Our system model consists of one client and one server. The server is assumed to be honest-but-curious, meaning that it will not inject malicious inputs to compromise the protocol, but can extract the information from the protocol transcript as much as possible. We assume that the client communicates with the server via a secure channel (e.g., TLS) in the synchronous model.
%
%We present the definition of DSSE as follows:
%
%\begin{definition}\label{def:DSSE}
%	A DSSE scheme is a tuple of one algorithm and two protocols $ \text{DSSE} = (\Gen,\Search,\Update) $
%	
%	\begin{enumerate}
%		\item $ (\I,\cib,\sigma,\K) \gets \Gen(1^\kappa,\fb) $: It takes as input a security parameter $ \kappa $, a list of (plaintext) documents and returns an encrypted index $ \I $, a list of encrypted files $ \cib $, a state $ \sigma $, and a key $ \K $ .
%		\item $ (\set{R},\sigma') \gets \Search_\K(w,\I,\sigma) $: The client inputs the key $ \K $, a keyword $ w $ to be searched, the server inputs the encrypted index $ \I $ and a state $ \sigma $. The protocol outputs the search result $ \set{R} $ to the client, and outputs a new state $ \sigma $ to the server.
%		\item $ (\I',\cib',\sigma') \gets \Update_\K(f,\I,\sigma,\cib) $: The client inputs the key $ \K $, a file to be updated $ f $, the servers inputs the encrypted index $ \I $, the state $ \sigma $ and the list of encrypted files $ \cib $. The protocol outputs to the server a newly updated encrypted index $ \I' $, the updated state $ \sigma' $, and the updated list of encrypted files $ \cib' $ where $ f $ is added or deleted.
%	\end{enumerate}
%\end{definition}
%In the following section, we present our proposed $ \ourdsse $ scheme according  to Definition \ref{def:DSSE}.
%%Describe the intuition of IM-DSSE here.








==> ARIS Arxiv/proposedschemes.tex <==
\section{The Proposed Scheme}\label{sec:proposedschemes}%

%%% SHIFT AND MERGE
\noindent {\it Intuition.} Our main observation is that the search query in standard DSSE reveals a part of the encrypted index to the server while retrieving the corresponding encrypted files. Therefore, once a keyword is searched again, it is not necessary to repeat the computation on the encrypted index to extract corresponding files that were previously revealed. Instead, one can leverage a more compact and simple data structure  (e.g., dictionary) to store file IDs revealed in the first search so that if the same query is repeated, the server will simply get the results stored in this data structure. This strategy will amortize the computation cost incurred in the first search operation and therefore, will make DSSE schemes more efficient. Note that the price to pay for gaining this search efficiency is (in worst case) doubling the server storage overhead. 

The second objective is to find a DSSE scheme that efficiently adopts the aforementioned strategy. We observe that, the DSSE scheme in \cite{DSSE:Yavuz:Archive:2015} offers a high level of security including forward-privacy with the cost of linear search complexity. This computation cost can be significantly reduced by using our proposed caching strategy mentioned above. Therefore, we take the DSSE scheme in $\cite{DSSE:Yavuz:Archive:2015} $ as the base case to construct $ \ourdsse $ with the caching strategy. We start by giving some brief overview about the data structures used in our scheme, some of which are borrowed from \cite{DSSE:Yavuz:Archive:2015}. We refer the reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description. Note that our caching strategy can be applied to {\em any forward-private DSSE scheme (e.g. Sophos~\cite{DSSE:Raphael:ForwardSecureSE})} to reduce the search cost.


\subsection{$ \ourdsse $ Data structures}
$ \ourdsse $ leverages three different types of data structure:
%Summary what kinds of data structures that we will use in this paper including
\subsubsection{Incidence matrix} Similar to \cite{DSSE:Yavuz:Archive:2015}, we construct the encrypted index using an incidence matrix $ \I $, which represents the keyword-file relationships via its cell values. Specifically, $ \I[i,j] =1 $ if the keyword indexing at row $i$ appears in the file indexing at column $ j $, and $ \I[i,j] =0 $ if otherwise. Search and update operations will access a row and a column of $ \I $, respectively. $ \I $ is encrypted bit-by-bit with IND-CPA encryption. Each cell of $ \I $ has a bit state as $ \I[i,j].st $ to keep track of the last access operation (search/update) on it. We refer reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description.
\subsubsection{Hash table} We use a hash table $ \TW $ to determine the row indexes assigned to the keywords in $ \I $. For simplicity, we assume files are indexed from 1 to $ \NumOfFiles $ and therefore, it is not required to create a hash table for them. In $ \TW $, we additionally store a counter for each keyword $ w $ as $ c_i \gets \TW[i].c $, where $i$ is the index of $w$ in $\TW$, which is incremented after each file update operation to achieve the forward-privacy. We refer reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description. We also store a state bit for each keyword $w$  in $\TW$ as $ v_i \gets\TW[i].v  $, which indicates if the keyword has just been searched ($v_i = 0$) or updated ($ v_i =1$). In $ \ourdsse $ scheme, we store $ \TW$  at the server, where all counters inside $ \TW $ are encrypted, to achieve $ \BigO{1} $ client storage, in which some of its components will be retrieved first during the search and update operations (see Section \ref{subsec:procedure}). 


%Since keywords may have different lengths and characteristics, they are indexed leveraging a hash table data structure and the search procedure is implemented using these indexes. Moreover, hash table offers $ \BigO{1}$ access time which is called frequently during our procedures.
%\NOTE{Talk about the hash table (at most 2 sentences).} 

\subsubsection{Dictionary}
$ \ourdsse $ leverages a caching strategy at the server to reduce the computation cost of repeated search operations. We employ a dictionary data structure $ D $ to store the search result of the queries when the keyword is first searched. $ D $ can be considered as an array of size $ m $, where $ D[i] $ stores the list of file IDs which is revealed when searching the keyword indexing at row $ i $ in $ \I $. $ D $ is encrypted with IND-CPA encryption and is updated if there are file operations performed on $ \I $ in between the search queries. We present the update policy in the following section to keep $ D $ consistent.


% We encrypt $ D $ with IND-CPA encryption. Of course, if there are update operations on $ \I $ between search operations, the array $ D $ will be updated with file IDs being added or deleted.    


%Given that there is an update between two search query



%We propose to add a cache data structure to store the search results at the server side after the first search. Since the results of the search are already revealed to the server, this structure does not leak any further information and offers in a amortized sub-linear search time. 

%This structure should be updated when an update procedure is called between two searches (see Section~\ref{subsec:procedure} for details), so we recommend to store a data structure with high-speed addition and deletion (e.g. dictionary) to store the cache. 
%\NOTE{Talk about the cache data structure (e.g., dictionary).  This is new in this paper so we should emphasize this. Try to expand to 3 sentences, and give the clear motivation why this is helpful here}

%Table 1 summarizes some notable notations that will be frequently used to describe our algorithms.




%\noindent \textbf{YG15~\cite{DSSE:Yavuz:Archive:2015}:} YG15 leverages very simple data structures such as bit matrix and hash tables for its design. Bit matrix is used to store keyword-file relations and hash tables are used for files and keywords separately. YG15 offers very high security properties (forward security and update size privacy) and still depends on symmetric key cryptography. (unlike some other schemes that depends on public key infrastructure such as Sophos~\cite{DSSE:Raphael:ForwardSecureSE}). Despite its pervasiveness, this scheme suffers from the linear search time that makes it unpractical for large databases.




%By leveraging a dictionary data structure along with the forward-private encrypted index used in \cite{DSSE:Yavuz:Archive:2015}, our scheme  propose a new DSSE scheme that offers (amortized) sub-linear search time and inherits all security advantages of the scheme in \cite{DSSE:Yavuz:Archive:2015} as outlined in Table \ref{table:AnalyticalComp}. 


%\noindent \textbf{Main Idea: }We notice that in all DSSE schemes, search operation leaks the information on the keyword-file pair relation for the given keyword, inevitably. Therefore, after one search on a keyword, server can store the file indexes that were returned for that keyword, without leaking any further information. Therefore, the cost of all future searches are highly reduced, in expense of storing a set for each keyword at the server side. With the increasing capabilities of servers and their storage sizes, we believe that this is a highly useful trade-off. This optimization enables us to have a sub-linear search time in average-case. Moreover, our search cost can be as low as O(1) some certain for use-cases, where search algorithm is invoked more frequently. 

%We further notice that our proposed scheme can get benefit of data structures in \ourdsse~\cite{DSSE:Yavuz:Archive:2015} to store file/keyword pairs. Therefore, we synergize incidence matrix structure to our optimization techniques to achieve an efficient yet secure scheme with easy design and implementation.

%Intuition: get rid of extra unnecessary encryptions and increasing counter (when server sees the index, no need to change the key for it). Therefore, only change the row key for update and add operations. Only update the encryption key with updating files. Make the search operation sub-linear by storing the indexes (the ones that are 1, meaning included in the file) for each row (keyword) in a $\langle$key,value$\rangle$ data structure where key is the keyword and value is the indexes? (Or maybe it can just store an array for keywords?). State bit will show us which cells were updated and then when search is made again for that keyword, just update the indexes of those cells in the dictionary (or array) data structure and return the files that are indexed in the data structure.

%\myedit{What if there are new keywords in the new added file? It seems like we can do this just by checking whether new keywords exist or not in previous ones generate new rows for new keywords where we set 0 all other files except the newly added one and encrypt those. However, does our algorithm handles it?}

%CONCERN: This way we do not show we are encrypting each cell with different keys, is this a problem? (ADD FILE COUNTER, Enrcypt with key file counter) Modification: We need to send new row keys to the server too (for updated files).


\subsection{Detailed $\ourdsse $ Procedures}\label{subsec:procedure}
In this section, we present the detailed procedures in $ \ourdsse $ according to Definition \ref{def:DSSE} as follows:\\
\vspace{-.7em}

\noindent \textbf{Setup: }First, given a list of plaintext files $ \fb $, the client creates the encrypted files $ \cib $ and encrypted index and sends them to the server by calling $\MainGen$ procedure. This procedure \textit{(i)} generates three keys, $\{\kf,\kt, \kd\}$ that collectively constitutes the key $ \K $, used to encrypt the files, the incidence matrix, and the counters in the hash table, respectively, \textit{(ii)} extracts keywords from the input files, each being assigned to a row index via the hash table $ \TW $, and \textit{(iii)} sets the corresponding value for each $ \I[i,j] $. Note that a counter for each keyword is also stored in $ \TW $, which will be used to derive a key to achieve the forward-privacy during update. Finally, the client generates the encrypted incidence matrix $\I$, encrypts counters in hash table $ \TW $ and encrypts all files $ \fb $, and sends them to the server, while keeping the key $ \K $ secret. % \NOTE{Counter is missing here, should store it in hash table, please see the Section IV.A.2}

\setlength{\textfloatsep}{6pt}% Remove \textfloatsep
\begin{figure}[t]
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				\Statex \hspace*{-1.8em} \underline{$(\I,\cib,\sigma,\K) \as \MainGen(1^{\kappa},\fb)$}: Create encrypted index
				
%				\noindent \textbf{Client: }
				
				\State $ \kf\as\Kg{1^{\kappa}} $ and $(\kt, \kd)\Ra\zo^{\kappa}$
				%\State $\K\as\{\kf,\kt,\kd\}$
				\State Set $ \K\as\{\kf,\kt, \kd\} $ 
				%\end{algorithmic}
				%	\algrule
				
				%\noindent	\textbf{Server: }
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(\I,\cib,\TW) \gets \MainSSEEnc_{\K}(\fb)$}
				\State Extract keywords $(\w_1,\ldots,\w_{\NumOfWords'})$ from $\fb=\{\f_{id_1},\ldots,\f_{id_{\NumOfFiles'}}\}$
				\State Set counter $u_i=1$, state $v_i=1$ for each $w_i$ in hash table $\TW$
				\State Set $\I[i,j] \as 1$ where $i$ is the keyword index in $\TW$ and $1 \le j \le \NumOfFiles $ if $\f_j$ contains keyword $i$
				\State Generate row keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $1\le i \le \NumOfWords$
				\State Encrypt each row of $\I$ with key $r_i$ for $1\le i \le \NumOfWords$ %\NOTE{and file index $j$???}
				\State Encrypt counters in hash table $\TW$ with $k_3$ 
%as $\I[i,j]\as \delta[i,j] \xor \HH{r_i||j||\ct_j}$ for $i=1,\ldots,\NumOfWords$ and  $j=1,\ldots,\NumOfFiles$
				\State Encrypt all files $\fb$ with $k_1$ as $\cib = \{c_j : c_j \gets \Enc{k_1}{f_j} \} $
				%\State Set $\sigma \as \TW$
				\State \Return $(\I,\cib,\sigma,\K)$, where $ \sigma \gets \TW$ (Send $(\I,\cib,\sigma)$ to server)
			\end{algorithmic}
	}}
\end{figure}


\begin{figure}[b]
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(i,r_i) \gets \MainSrchToken{(\K,\w)}$}
				\Statex \hspace*{-1.8em} \underline{$ (\set{R},\sigma') \as \MainSearch_\K(w,\I,\sigma) $}
				
				\noindent \hspace{-1.8em} \textbf{Client: }
				\State Let $i$ be index of $w$ in $ \TW $
				\State Download the counter $u_i$ of keyword $\w_i$ in $\TW$
%				\State Request and get the encrypted index corresp. to keyword $\w$ from the server using the hash value
%				\State Decrypt the encrypted index as $i$
				\State Decrypt  $u_i$ with $k_3$ and generate key $r_i\as \mathsf{PRF}(\kt||i||u_i)$
%				\State \NOTE{Set the state $v'_i$ to 1 and encrypt it} 
				\State Send $(i,v'_i,r_i)$ to server
				%\end{algorithmic}
				%	\algrule
				
				\noindent \hspace{-1.8em} \textbf{Server:}  On receive $(i,v'_i,r_i)$: 
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$ (D[i], \cib_w) \as \MainSearch(i,r_i) $}
%				\State \NOTE{Update $\TW$ with $v'_i$}
				\If{$i$ is first-time searched}
				%\State Decrypt $\I[i,*]$ with the 
				\State Let $\I'[i,*]$ be the decryption of $\I[i,*]$ using key $r_i$
				\State $D[i] \as \{j: \I'[i,j]=1\}$
				%\State Deterministically generate secret key to encrypt $D[i]$
				\State Encrypt $D[i]$
				\Else
				\State Decrypt $D[i]$ %with row key $r_i$
				\State Let $J = \{ j: \I[i,j].st = 1\}$
				\For{each $j$ in $J$}
				\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$ using key $ r_i $ 
				%	\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$
				\State Add $j$ to $D[i]$ if $\I'[i,j] = 1$, or delete $j$ if otherwise
				%	\State Delete $j$ from $D[i]$ if $\I'[i,j] \neq 1$
				\EndFor
				\EndIf
				\State Send $\set{R} = \{ c_j : j \in D[i] \}$  to client 
				\State Re-encrypt $D[i]$, set $\I[i,*].st = 0$ and $\TW[i].v \gets 0$
				%\State $\sigma' \gets \TW$
				%
				\State \Return $(\set{R},\sigma') $, where $ \sigma' \gets \TW $  with $i$-th entry being updated
				%\end{algorithmic}
				
				\noindent \hspace{-1.8em} \textbf{Client: } On receive $\set{R}$:
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$\f \gets \MainSSEDec_{\K}{(c)}$}
				\State $\f_j\as\Dec{\kf}{c_j}$ for each $c_j \in \set{R}$ %where $u$ is the file counter and $y$ is column index
				%\State \Return $ \f$
			\end{algorithmic}
			%	\algrule
	}}\vspace{-3mm}
\end{figure}

\noindent \textbf{Search:} To search a keyword $ w $, the client first requests the encrypted counter of $ w $ stored in $ \TW $. Then, they send a search token containing the row index $ i $ and the row key $ r_i $ derived from the counter, to the server. If the keyword is being searched for the first time, then the server decrypts the whole row $\I[i,*]$ with $ r_i $, adds all column indexes $ j $, where $ \I[i,j] =1 $, to the dictionary $D[i]$, and encrypts $ D[i] $\footnote{Server encrypts D with a self-generated key just to preserve the data privacy against outside attackers.}. The server returns the corresponding encrypted files matching with such indexes to the client.


If a previously-searched keyword is searched again, the server retrieves indexes of corresponding encrypted files by simply decrypting $D[i]$. It is important to note that $ D[i] $ might need to be updated, given that there are some file update operations on $ \I $ that happened after the latest search on $ w_i $. This is achieved by checking the state bit $\I[*,*].st $. Specifically, if $ \I[i,j].st = 1 $, then the server decrypts $\I[i,j]$ and adds the entry $ j $ to $ D[i] $ if $ \I[i,j] = 1$ (or deletes $ j $ if $ \I[i,j] = 0 $).

%  changed in between two searches. Specifically, if the database is updated, the dictionary $D[i]$ should also be updated. 
  
  
%  Therefore, at this step, we need to check the states of each cell, to see if the last operation on it was search, or update. Every updated cell should be decrypted and the dictionary should also be updated accordingly. However, if the last operation was search, this means dictionary is up-to-date for that cell, and we do not need to decrypt these cells.  %\NOTE{talk about if there is update sequence here, VERY IMPORTANT, please make it clear and expanded!}
 
The use of data structure $ D $ enables $ \ourdsse $ to have an amortized sublinear search complexity. Specifically, the computation cost of the first query is $ \BigO{\NumOfFiles} $ while that of repeated queries is $ \BigO{r} $, where $ r  $ is the result size of the first query. The amortized cost is $\BigO{{r + d_w}}$, where $d_w$ is the number of updates, after $ \NumOfFiles $ search repetitions. \\ % \NOTE{ give the equation sum of two BigO above here}.\\
 
%  One may notice that the cost of search operation is highly reduced in expense of storing a set of file indexes for each keyword at the server side. After the first search on the keyword, the cost is decreased to {\em size of encrypted dictionary and the number of updates on distinct files}. Therefore, our search algorithm has amortized sub-linear overhead.\\
\vspace{-.7em}

\noindent \textbf{Update: } Given an updated file $ f_j $, the client extracts the updated keywords and creates an unencrypted column $\I[*,j]$, which represents the relationship between $ f_j $ with all the keywords in DB. The client then generates $\NumOfWords$ row keys $r_i$ according to corresponding counters stored in  $\TW$ at the server. To achieve the forward-privacy, the client must encrypt $\I[*,j]$ with fresh keys, which are unknown to the server. This can be done by generating the row key with the incremental counter, given that the key generated with the current counter has been previously revealed to the server during the previous searches. Finally, the client sends the encrypted column and the encrypted files to the server, where the encrypted index and encrypted database are updated accordingly.


\begin{figure}[h]
	\
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(\mat{\II}, c, j)\as \MainUpdateToken(\K,f_j)$}
				\Statex \hspace*{-1.8em}\underline{$(\I',\cib',\sigma') \as \MainUpdate_\K(f_j,\I,\sigma,\cib)$}
				%\State \myedit{Identify the changed cells and increase the counter for them only, at least for update} 
				
				\noindent \hspace{-1.8em} \textbf{Client: }
				
				\State Set $\mat{\II}[*,j]\as0$ and $c \as NULL$
				\State Download all counters $u_i$ and states $v_i$ ($1\le i\le\NumOfWords$) in $\TW$
				\State Download state column $\I[*,j].\st$
				\State Let $V = \{ i: v_i = 0\}$
				\State Extract keywords $(w_1,\ldots,w_t)$ from $\f_{j}$
				\State Decrypt counters $u_i$ with $k_3$, and set $u_i \gets u_i+1$ for each $i \in V$
				\State Generate keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ %\NOTE{for each $i \in V$} %\myedit{Where did counter came from, client should not store it}
				%\If{Operation is Add/Update/Replace}
				\State Set $\mat{\II}[{x_i},j]\as1$ for $1\le i \le t$, where $x_i$ is index of $w_i$ in $\TW$
				\State Encrypt $f_j$ as $ c_j  \gets \Enc{\kf}{\f_{j}}$
				%\EndIf
				%	\State Set $\I[*,j].st = 1 $ 
				\State Encrypt each row $\mat{\II}[i,j]$ with row keys $r_i$, for $1 \le i \le \NumOfWords$ %\NOTE{and file index $j$???}
				%\State Set $v_i = 0$ for each $i \in V$
				\State Let $\vec{u} \gets (u_1,\dots,u_\NumOfFiles)$, where each $u_i$ is encrypted with $k_3$
				\State Send $(\mat{\II}[*,j], c_j, j, \vec{u})$ to server
				%\end{algorithmic}
				%	\algrule
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em}\underline{$(\I,\cib) \as \MainUpdate(\I,\cib,\mat{\II}, c, j)$}
				
				\noindent \hspace{-1.8em} \textbf{Server: } On receive $(\mat{\II}[*,j], c_j, j, \vec{u})$:
				
				\State $\TW[i].u \gets u_i$ and set $\TW[i].v \gets 1$ for $1 \le i \le \NumOfWords$
				\State  Set $\I[*,j]\as\mat{\II}[*,j] $ and $\I[*,j].\st\as 1$ %, for $ 1 \le i \le \NumOfWords $ %and  $0 \le j \le \NumOfFiles $ \NOTE{We might discuss this but all the revealed row keys are updated so I think state should be set to 1 for all matrix}
				%	\State $\TF[j].\ctht$ $\as \TF[j].\ctht+1$
				%\State Update $\cib$ with $c_j$
				%\If {c is $NULL$}
				\State \Return $(\I',\cib',\sigma')$, where $\I' = \I$ with column $j$ updated, $\cib' = \cib$ updated with $c_j$, $\sigma' = \TW $ with counters and states updated % \gets \cib \cup \{(c,j)\}$ 
				%\Else
				%\State \Return $(\I,\cib',\sigma')$, $\cib' \gets \cib \setminus \{(c,j)\}$ 
				%\EndIf
				
			\end{algorithmic}
	}}
\vspace{-3mm}
\end{figure}

% \NOTE{}
% Row counters are increased if the row key was revealed to the server (i.e. last operation on the cell was search). Revealed row keys are re-generated and the column is encrypted with these keys. 
 
% Encrypted 
% 
% column is sent along with the ciphertext of file and the encrypted row indexes. Server only adds the new file to the database (or extract if operation is delete), updates the column j in encrypted matrix and updates the encrypted counter in $\TW$.


%\NOTE{Present according to intuitive step-by-step instruction style, like the one that I gave in the Search, but be GENERAL! For example, Given a file to be updated $ f $ -> extract keywords to be updated-> create unecencrypted column, get the row counter of these keywords from hash table TW from the server -> increase the counter -> generate row keys -> encrypt the column with these keys -> send it along with the ciphertext of file to server, and sends all encrypted updated row counters to server -> server update the column j and the encrypted counter in $ TW $. }




%Moreover, client increases the counter for row key generation and encrypts the column for incident matrix with new row keys (if the key was seen by server in a previous search query) to preserve forward security. Server just replaces the jth column of the incident matrix with the column in token, and adds/deletes the encrypted file to/from the database.


%Note that row keys are updated with the invocation of Update algorithm to provide forward security. %However, as search operation reveals the key, there is no need to increase the counter and change the row keys.



%\begin{scheme}{1}{!b}
%	\floatname{algorithm}{Proposed Scheme}
%	\caption{$ DSSE $ scheme}\label{scheme:DSSE}
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$\K \as \MainGen(1^{\kappa})$}
%		\State $ \kf\as\Kg{1^{\kappa}} $ and $(\kt)\Ra\zo^{\kappa}$
%		%\State $\K\as\{\kf,\kt,\kd\}$
%		\State \Return $ \K $, where $ \K\as\{\kf,\kt\} $ 
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$\f \gets \MainSSEDec_{\K}{(c)}$}
%		\State $\f\as\Dec{\kf}{c,y||\ct}$ %where $u$ is the file counter and $y$ is column index
%		\State \Return $ \f$
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(\I,\cib) \gets \MainSSEEnc_{\K}(\fb)$}
%		\State Extract keywords $(\w_1,\ldots,\w_{\NumOfWords'})$ from files $\fb=\{\f_{id_1},\ldots,\f_{id_{\NumOfFiles'}}\}$
%		\State Add all keywords to hash table $\TW$
%		\State Set $\I[i,j] \as 1$ where $i$ is the index of keywords in $\TW$ and $0 \le j \le \NumOfFiles $ if $\f_j$ contains keyword $i$
%		\State Generate row keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $i=1,\ldots,\NumOfWords$
%		\State Encrypt each row of $\I$ with row key $r_i$ %as $\I[i,j]\as \delta[i,j] \xor \HH{r_i||j||\ct_j}$ for $i=1,\ldots,\NumOfWords$ and  $j=1,\ldots,\NumOfFiles$
%		\State Let $\cib$ be the set of files encrypted by $k_1$
%		\State \Return $(\I,\cib)$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(i,r_i) \gets \MainSrchToken{(\K,\w)}$}
%		\State Get the index $i$ for the keyword from $\TW$
%		\State Generate the search token for the keyword with index $i$, $r_i\as \mathsf{PRF}(\kt||i||u_i)$ 
%		\State \Return $(i,r_i)$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$ (D[i], \cib_w) \as \MainSearch((i,r_i),\gamma) $}
%		\If{It is the 1st search on $i$}
%		\State Decrypt $\I[i,*]$ with the key $r_i$
%		\State Let $\I'[i,*]$ be the decryption of $\I[i,*]$
%		\State $D[i] \as \{j: \I'[i,j]=1\}$
%		\State Encrypt $D[i]$ with row key $r_i$
%		\Else
%		\State Decrypt $\I[i,j]$ such that $\I[i,j].st = 1$
%		\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$
%		\State Decrypt $D[i]$ with row key $r_i$
%		\State Add $j$ to $D[i]$ if $\I'[i,j] = 1$
%		\State Delete $j$ from $D[i]$ if $\I'[i,j] \neq 1$
%		\State Re-Encrypt $D[i]$ with row key $r_i$
%		\EndIf
%		
%		%	\State Check if there is a stored $\idw$ for row id $i$ 
%		%	
%		%	\If {$|\idw| \neq 0$}
%		%	
%		%	\If {$\I[i,j].\st = 1$ for $j=1,\ldots,\NumOfFiles$}
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 1$ and j is not in $\idw$}
%		%	\State Add j to $\idw$
%		%	\EndIf
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 0$ and j is in $\idw$}
%		%	\State Extract j from $\idw$
%		%	\EndIf
%		%	\State Set $\I[i,j].\st \as 0$
%		%	\EndIf
%		%	\EndIf
%		%	\If {$|\idw| = 0$ (first search on keywords $w$)}
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 1$ for $j=1,\ldots,\NumOfFiles$}
%		%	\State Add j to $\idw$
%		%	\EndIf
%		%	\EndIf
%		\State Set $\cib_w$ as encrypted files corresp. to the indexes in $D[i]$
%		\State \Return $ (D[i],\cib_w) $ (Send to client)
%	\end{algorithmic}
%	%	\algrule
%	
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(\mat{\II}, c, j)\as \MainUpdateToken(\K,f_j)$}
%		%\State \myedit{Identify the changed cells and increase the counter for them only, at least for update} 
%		\State Set $\mat{\II}[*,j]\as0$ and $c \as NULL$
%		\If{Operation is Add/Update/Replace}
%		\State Extract keywords $(w_1,\ldots,w_t)$ from file $\f_{j}$
%		\State Increase the row counter $u_i$ by 1 and re-generate all row keys  $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $i=1,\ldots,\NumOfWords$
%		\State Set $\mat{\II}[x_i,j]\as1$ for $i=1,\ldots,t$
%		\State Encrypt the file as $c \gets \Enc{\kf}{\f_{id},j||\ct_j}$
%		\EndIf
%		\State Encrypt $\mat{\II}$ with row key $r_i$
%		\State \Return $\mat{\II}, c, j$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em}\underline{$(\I,\cib) \as \MainUpdate(\I,\cib,\mat{\II}, c, j)$}
%		\State  Set $\I[i,j]\as\mat{\II}[i,j] $ and $\I[i,j].\st\as 1$, for $ 1 \le i \le \NumOfWords $
%		%	\State $\TF[j].\ctht$ $\as \TF[j].\ctht+1$
%		\If {c is $NULL$}
%		\State \Return $(\I,\cib)$, $\cib' \gets \cib \cup \{(c,j)\}$ (Send to client)
%		\Else
%		\State \Return $(\I,\cib)$, $\cib' \gets \cib \setminus \{(c,j)\}$ (Send to client)
%		\EndIf
%		
%	\end{algorithmic}
%\end{scheme}







==> ARIS Arxiv/related.tex <==
\section{Related Work}\label{sec:related}
 
 One-time signatures (e.g. HORS \cite{HORS_BetterthanBiBa02})  have been proposed to offer fast signing and verification.  Following HORS,  many schemes with different performance and security trade-offs such as time valid one-time signatures (i.e., TV-HORS  \cite{TVHORSInfocom09}) have been proposed. However, these schemes suffer from security and performance penalties incurred due to the need for time-synchronization and their low tolerance for packet loss.  Multiple-time hash-based signatures (e.g., XMSS \cite{XMSS:Buchmann:2011}) utilize Merkle-Tree and can sign multiple messages by keeping the signer's state. Recently, stateless variations (e.g., SPHINCS  \cite{SPHINCS}) have been proposed, however such schemes suffer from large signatures ($ \approx $ 41 KB) and slow signing algorithms.  
% 
% The continuous renewal and certification of the new keys might be impractical. \myedit{a few sentence for their multi-ptime variants SPHINCS and XMSS etc., discuss TV-HORS seperately, there are fans of it}. 

%There has been many attempts to propose new methods or efficient implementations to push the limits of  signature schemes. 
Recently, a polynomially-bounded multiple-time signature scheme based on HORS design  is proposed \cite{Tachyon}.  The scheme utilizes the additive homomorphic property of the underlying one-way function to obtain fast signatures  where the signer only aggregates private key components  during the online phase.  However, despite its   efficiency,  it cannot meet the stringent delay requirement of some IoT applications. 
%Some methods rely on shifting the   computation extensive operations to the key generation algorithms~\cite{OfflineOnline_ImprovedShamir_2001}. For instance, the Rapid Authentication scheme proposed in \cite{RA:Yavuz} exploits the aggregatable property of the underlying signature schemes and obtains  fast signature generation where the signer only aggregates tokens (i.e., signatures of the underlying scheme) during the online phase that are precomputed in the key generation  (offline). However, RA requires messages to be in a predefined and fixed-length format.  
Another  proposed scheme called CEDA \cite{CEDA}  exploits the aggregatable property of RSA-based one-way permutation functions and message encoding (as proposed in \cite{HORS_BetterthanBiBa02}) to  attain efficient signing. However, the large parameter sizes not only incur very large public keys but also make the  exponentiations that takes place during signature generation and verification quite costly. Therefore CEDA, while being among the most efficient schemes, does not surpass the latest implementations of signatures on fast elliptic curves. 

In the line of  proposing fast elliptic curves, Renes et al. \cite{Kummer} presented an  efficient instantiations of  the scheme in \cite{Ed25519} based on Kummer surface that shows significant performance gains as compared to its base scheme \cite{Ed25519}.   In 2016, Costello et al.  \cite{SchnorrQ} proposed a new implementation of  \cite{Ed25519} based on another  elliptic curve called  FourQ  which shows to even outperform the implementation in  \cite{Kummer}.   

==> proposedschemes.tex <==
\section{The Proposed Scheme}\label{sec:proposedschemes}%

%%% SHIFT AND MERGE
\noindent {\it Intuition.} Our main observation is that the search query in standard DSSE reveals a part of the encrypted index to the server while retrieving the corresponding encrypted files. Therefore, once a keyword is searched again, it is not necessary to repeat the computation on the encrypted index to extract corresponding files that were previously revealed. Instead, one can leverage a more compact and simple data structure  (e.g., dictionary) to store file IDs revealed in the first search so that if the same query is repeated, the server will simply get the results stored in this data structure. This strategy will amortize the computation cost incurred in the first search operation and therefore, will make DSSE schemes more efficient. Note that the price to pay for gaining this search efficiency is (in worst case) doubling the server storage overhead. 

The second objective is to find a DSSE scheme that efficiently adopts the aforementioned strategy. We observe that, the DSSE scheme in \cite{DSSE:Yavuz:Archive:2015} offers a high level of security including forward-privacy with the cost of linear search complexity. This computation cost can be significantly reduced by using our proposed caching strategy mentioned above. Therefore, we take the DSSE scheme in $\cite{DSSE:Yavuz:Archive:2015} $ as the base case to construct $ \ourdsse $ with the caching strategy. We start by giving some brief overview about the data structures used in our scheme, some of which are borrowed from \cite{DSSE:Yavuz:Archive:2015}. We refer the reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description. Note that our caching strategy can be applied to {\em any forward-private DSSE scheme (e.g. Sophos~\cite{DSSE:Raphael:ForwardSecureSE})} to reduce the search cost.


\subsection{$ \ourdsse $ Data structures}
$ \ourdsse $ leverages three different types of data structure:
%Summary what kinds of data structures that we will use in this paper including
\subsubsection{Incidence matrix} Similar to \cite{DSSE:Yavuz:Archive:2015}, we construct the encrypted index using an incidence matrix $ \I $, which represents the keyword-file relationships via its cell values. Specifically, $ \I[i,j] =1 $ if the keyword indexing at row $i$ appears in the file indexing at column $ j $, and $ \I[i,j] =0 $ if otherwise. Search and update operations will access a row and a column of $ \I $, respectively. $ \I $ is encrypted bit-by-bit with IND-CPA encryption. Each cell of $ \I $ has a bit state as $ \I[i,j].st $ to keep track of the last access operation (search/update) on it. We refer reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description.
\subsubsection{Hash table} We use a hash table $ \TW $ to determine the row indexes assigned to the keywords in $ \I $. For simplicity, we assume files are indexed from 1 to $ \NumOfFiles $ and therefore, it is not required to create a hash table for them. In $ \TW $, we additionally store a counter for each keyword $ w $ as $ c_i \gets \TW[i].c $, where $i$ is the index of $w$ in $\TW$, which is incremented after each file update operation to achieve the forward-privacy. We refer reader to \cite{DSSE:Yavuz:Archive:2015} for detailed description. We also store a state bit for each keyword $w$  in $\TW$ as $ v_i \gets\TW[i].v  $, which indicates if the keyword has just been searched ($v_i = 0$) or updated ($ v_i =1$). In $ \ourdsse $ scheme, we store $ \TW$  at the server, where all counters inside $ \TW $ are encrypted, to achieve $ \BigO{1} $ client storage, in which some of its components will be retrieved first during the search and update operations (see Section \ref{subsec:procedure}). 


%Since keywords may have different lengths and characteristics, they are indexed leveraging a hash table data structure and the search procedure is implemented using these indexes. Moreover, hash table offers $ \BigO{1}$ access time which is called frequently during our procedures.
%\NOTE{Talk about the hash table (at most 2 sentences).} 

\subsubsection{Dictionary}
$ \ourdsse $ leverages a caching strategy at the server to reduce the computation cost of repeated search operations. We employ a dictionary data structure $ D $ to store the search result of the queries when the keyword is first searched. $ D $ can be considered as an array of size $ m $, where $ D[i] $ stores the list of file IDs which is revealed when searching the keyword indexing at row $ i $ in $ \I $. $ D $ is encrypted with IND-CPA encryption and is updated if there are file operations performed on $ \I $ in between the search queries. We present the update policy in the following section to keep $ D $ consistent.


% We encrypt $ D $ with IND-CPA encryption. Of course, if there are update operations on $ \I $ between search operations, the array $ D $ will be updated with file IDs being added or deleted.    


%Given that there is an update between two search query



%We propose to add a cache data structure to store the search results at the server side after the first search. Since the results of the search are already revealed to the server, this structure does not leak any further information and offers in a amortized sub-linear search time. 

%This structure should be updated when an update procedure is called between two searches (see Section~\ref{subsec:procedure} for details), so we recommend to store a data structure with high-speed addition and deletion (e.g. dictionary) to store the cache. 
%\NOTE{Talk about the cache data structure (e.g., dictionary).  This is new in this paper so we should emphasize this. Try to expand to 3 sentences, and give the clear motivation why this is helpful here}

%Table 1 summarizes some notable notations that will be frequently used to describe our algorithms.




%\noindent \textbf{YG15~\cite{DSSE:Yavuz:Archive:2015}:} YG15 leverages very simple data structures such as bit matrix and hash tables for its design. Bit matrix is used to store keyword-file relations and hash tables are used for files and keywords separately. YG15 offers very high security properties (forward security and update size privacy) and still depends on symmetric key cryptography. (unlike some other schemes that depends on public key infrastructure such as Sophos~\cite{DSSE:Raphael:ForwardSecureSE}). Despite its pervasiveness, this scheme suffers from the linear search time that makes it unpractical for large databases.




%By leveraging a dictionary data structure along with the forward-private encrypted index used in \cite{DSSE:Yavuz:Archive:2015}, our scheme  propose a new DSSE scheme that offers (amortized) sub-linear search time and inherits all security advantages of the scheme in \cite{DSSE:Yavuz:Archive:2015} as outlined in Table \ref{table:AnalyticalComp}. 


%\noindent \textbf{Main Idea: }We notice that in all DSSE schemes, search operation leaks the information on the keyword-file pair relation for the given keyword, inevitably. Therefore, after one search on a keyword, server can store the file indexes that were returned for that keyword, without leaking any further information. Therefore, the cost of all future searches are highly reduced, in expense of storing a set for each keyword at the server side. With the increasing capabilities of servers and their storage sizes, we believe that this is a highly useful trade-off. This optimization enables us to have a sub-linear search time in average-case. Moreover, our search cost can be as low as O(1) some certain for use-cases, where search algorithm is invoked more frequently. 

%We further notice that our proposed scheme can get benefit of data structures in \ourdsse~\cite{DSSE:Yavuz:Archive:2015} to store file/keyword pairs. Therefore, we synergize incidence matrix structure to our optimization techniques to achieve an efficient yet secure scheme with easy design and implementation.

%Intuition: get rid of extra unnecessary encryptions and increasing counter (when server sees the index, no need to change the key for it). Therefore, only change the row key for update and add operations. Only update the encryption key with updating files. Make the search operation sub-linear by storing the indexes (the ones that are 1, meaning included in the file) for each row (keyword) in a $\langle$key,value$\rangle$ data structure where key is the keyword and value is the indexes? (Or maybe it can just store an array for keywords?). State bit will show us which cells were updated and then when search is made again for that keyword, just update the indexes of those cells in the dictionary (or array) data structure and return the files that are indexed in the data structure.

%\myedit{What if there are new keywords in the new added file? It seems like we can do this just by checking whether new keywords exist or not in previous ones generate new rows for new keywords where we set 0 all other files except the newly added one and encrypt those. However, does our algorithm handles it?}

%CONCERN: This way we do not show we are encrypting each cell with different keys, is this a problem? (ADD FILE COUNTER, Enrcypt with key file counter) Modification: We need to send new row keys to the server too (for updated files).


\subsection{Detailed $\ourdsse $ Procedures}\label{subsec:procedure}
In this section, we present the detailed procedures in $ \ourdsse $ according to Definition \ref{def:DSSE} as follows:\\
\vspace{-.7em}

\noindent \textbf{Setup: }First, given a list of plaintext files $ \fb $, the client creates the encrypted files $ \cib $ and encrypted index and sends them to the server by calling $\MainGen$ procedure. This procedure \textit{(i)} generates three keys, $\{\kf,\kt, \kd\}$ that collectively constitutes the key $ \K $, used to encrypt the files, the incidence matrix, and the counters in the hash table, respectively, \textit{(ii)} extracts keywords from the input files, each being assigned to a row index via the hash table $ \TW $, and \textit{(iii)} sets the corresponding value for each $ \I[i,j] $. Note that a counter for each keyword is also stored in $ \TW $, which will be used to derive a key to achieve the forward-privacy during update. Finally, the client generates the encrypted incidence matrix $\I$, encrypts counters in hash table $ \TW $ and encrypts all files $ \fb $, and sends them to the server, while keeping the key $ \K $ secret. % \NOTE{Counter is missing here, should store it in hash table, please see the Section IV.A.2}

\setlength{\textfloatsep}{6pt}% Remove \textfloatsep
\begin{figure}[t]
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				\Statex \hspace*{-1.8em} \underline{$(\I,\cib,\sigma,\K) \as \MainGen(1^{\kappa},\fb)$}: Create encrypted index
				
%				\noindent \textbf{Client: }
				
				\State $ \kf\as\Kg{1^{\kappa}} $ and $(\kt, \kd)\Ra\zo^{\kappa}$
				%\State $\K\as\{\kf,\kt,\kd\}$
				\State Set $ \K\as\{\kf,\kt, \kd\} $ 
				%\end{algorithmic}
				%	\algrule
				
				%\noindent	\textbf{Server: }
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(\I,\cib,\TW) \gets \MainSSEEnc_{\K}(\fb)$}
				\State Extract keywords $(\w_1,\ldots,\w_{\NumOfWords'})$ from $\fb=\{\f_{id_1},\ldots,\f_{id_{\NumOfFiles'}}\}$
				\State Set counter $u_i=1$, state $v_i=1$ for each $w_i$ in hash table $\TW$
				\State Set $\I[i,j] \as 1$ where $i$ is the keyword index in $\TW$ and $1 \le j \le \NumOfFiles $ if $\f_j$ contains keyword $i$
				\State Generate row keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $1\le i \le \NumOfWords$
				\State Encrypt each row of $\I$ with key $r_i$ for $1\le i \le \NumOfWords$ %\NOTE{and file index $j$???}
				\State Encrypt counters in hash table $\TW$ with $k_3$ 
%as $\I[i,j]\as \delta[i,j] \xor \HH{r_i||j||\ct_j}$ for $i=1,\ldots,\NumOfWords$ and  $j=1,\ldots,\NumOfFiles$
				\State Encrypt all files $\fb$ with $k_1$ as $\cib = \{c_j : c_j \gets \Enc{k_1}{f_j} \} $
				%\State Set $\sigma \as \TW$
				\State \Return $(\I,\cib,\sigma,\K)$, where $ \sigma \gets \TW$ (Send $(\I,\cib,\sigma)$ to server)
			\end{algorithmic}
	}}
\end{figure}


\begin{figure}[b]
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(i,r_i) \gets \MainSrchToken{(\K,\w)}$}
				\Statex \hspace*{-1.8em} \underline{$ (\set{R},\sigma') \as \MainSearch_\K(w,\I,\sigma) $}
				
				\noindent \hspace{-1.8em} \textbf{Client: }
				\State Let $i$ be index of $w$ in $ \TW $
				\State Download the counter $u_i$ of keyword $\w_i$ in $\TW$
%				\State Request and get the encrypted index corresp. to keyword $\w$ from the server using the hash value
%				\State Decrypt the encrypted index as $i$
				\State Decrypt  $u_i$ with $k_3$ and generate key $r_i\as \mathsf{PRF}(\kt||i||u_i)$
%				\State \NOTE{Set the state $v'_i$ to 1 and encrypt it} 
				\State Send $(i,v'_i,r_i)$ to server
				%\end{algorithmic}
				%	\algrule
				
				\noindent \hspace{-1.8em} \textbf{Server:}  On receive $(i,v'_i,r_i)$: 
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$ (D[i], \cib_w) \as \MainSearch(i,r_i) $}
%				\State \NOTE{Update $\TW$ with $v'_i$}
				\If{$i$ is first-time searched}
				%\State Decrypt $\I[i,*]$ with the 
				\State Let $\I'[i,*]$ be the decryption of $\I[i,*]$ using key $r_i$
				\State $D[i] \as \{j: \I'[i,j]=1\}$
				%\State Deterministically generate secret key to encrypt $D[i]$
				\State Encrypt $D[i]$
				\Else
				\State Decrypt $D[i]$ %with row key $r_i$
				\State Let $J = \{ j: \I[i,j].st = 1\}$
				\For{each $j$ in $J$}
				\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$ using key $ r_i $ 
				%	\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$
				\State Add $j$ to $D[i]$ if $\I'[i,j] = 1$, or delete $j$ if otherwise
				%	\State Delete $j$ from $D[i]$ if $\I'[i,j] \neq 1$
				\EndFor
				\EndIf
				\State Send $\set{R} = \{ c_j : j \in D[i] \}$  to client 
				\State Re-encrypt $D[i]$, set $\I[i,*].st = 0$ and $\TW[i].v \gets 0$
				%\State $\sigma' \gets \TW$
				%
				\State \Return $(\set{R},\sigma') $, where $ \sigma' \gets \TW $  with $i$-th entry being updated
				%\end{algorithmic}
				
				\noindent \hspace{-1.8em} \textbf{Client: } On receive $\set{R}$:
				
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$\f \gets \MainSSEDec_{\K}{(c)}$}
				\State $\f_j\as\Dec{\kf}{c_j}$ for each $c_j \in \set{R}$ %where $u$ is the file counter and $y$ is column index
				%\State \Return $ \f$
			\end{algorithmic}
			%	\algrule
	}}\vspace{-3mm}
\end{figure}

\noindent \textbf{Search:} To search a keyword $ w $, the client first requests the encrypted counter of $ w $ stored in $ \TW $. Then, they send a search token containing the row index $ i $ and the row key $ r_i $ derived from the counter, to the server. If the keyword is being searched for the first time, then the server decrypts the whole row $\I[i,*]$ with $ r_i $, adds all column indexes $ j $, where $ \I[i,j] =1 $, to the dictionary $D[i]$, and encrypts $ D[i] $\footnote{Server encrypts D with a self-generated key just to preserve the data privacy against outside attackers.}. The server returns the corresponding encrypted files matching with such indexes to the client.


If a previously-searched keyword is searched again, the server retrieves indexes of corresponding encrypted files by simply decrypting $D[i]$. It is important to note that $ D[i] $ might need to be updated, given that there are some file update operations on $ \I $ that happened after the latest search on $ w_i $. This is achieved by checking the state bit $\I[*,*].st $. Specifically, if $ \I[i,j].st = 1 $, then the server decrypts $\I[i,j]$ and adds the entry $ j $ to $ D[i] $ if $ \I[i,j] = 1$ (or deletes $ j $ if $ \I[i,j] = 0 $).

%  changed in between two searches. Specifically, if the database is updated, the dictionary $D[i]$ should also be updated. 
  
  
%  Therefore, at this step, we need to check the states of each cell, to see if the last operation on it was search, or update. Every updated cell should be decrypted and the dictionary should also be updated accordingly. However, if the last operation was search, this means dictionary is up-to-date for that cell, and we do not need to decrypt these cells.  %\NOTE{talk about if there is update sequence here, VERY IMPORTANT, please make it clear and expanded!}
 
The use of data structure $ D $ enables $ \ourdsse $ to have an amortized sublinear search complexity. Specifically, the computation cost of the first query is $ \BigO{\NumOfFiles} $ while that of repeated queries is $ \BigO{r} $, where $ r  $ is the result size of the first query. The amortized cost is $\BigO{{r + d_w}}$, where $d_w$ is the number of updates, after $ \NumOfFiles $ search repetitions. \\ % \NOTE{ give the equation sum of two BigO above here}.\\
 
%  One may notice that the cost of search operation is highly reduced in expense of storing a set of file indexes for each keyword at the server side. After the first search on the keyword, the cost is decreased to {\em size of encrypted dictionary and the number of updates on distinct files}. Therefore, our search algorithm has amortized sub-linear overhead.\\
\vspace{-.7em}

\noindent \textbf{Update: } Given an updated file $ f_j $, the client extracts the updated keywords and creates an unencrypted column $\I[*,j]$, which represents the relationship between $ f_j $ with all the keywords in DB. The client then generates $\NumOfWords$ row keys $r_i$ according to corresponding counters stored in  $\TW$ at the server. To achieve the forward-privacy, the client must encrypt $\I[*,j]$ with fresh keys, which are unknown to the server. This can be done by generating the row key with the incremental counter, given that the key generated with the current counter has been previously revealed to the server during the previous searches. Finally, the client sends the encrypted column and the encrypted files to the server, where the encrypted index and encrypted database are updated accordingly.


\begin{figure}[h]
	\
	\noindent\fbox{\parbox{0.97\linewidth}{
			\small
			\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em} \underline{$(\mat{\II}, c, j)\as \MainUpdateToken(\K,f_j)$}
				\Statex \hspace*{-1.8em}\underline{$(\I',\cib',\sigma') \as \MainUpdate_\K(f_j,\I,\sigma,\cib)$}
				%\State \myedit{Identify the changed cells and increase the counter for them only, at least for update} 
				
				\noindent \hspace{-1.8em} \textbf{Client: }
				
				\State Set $\mat{\II}[*,j]\as0$ and $c \as NULL$
				\State Download all counters $u_i$ and states $v_i$ ($1\le i\le\NumOfWords$) in $\TW$
				\State Download state column $\I[*,j].\st$
				\State Let $V = \{ i: v_i = 0\}$
				\State Extract keywords $(w_1,\ldots,w_t)$ from $\f_{j}$
				\State Decrypt counters $u_i$ with $k_3$, and set $u_i \gets u_i+1$ for each $i \in V$
				\State Generate keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ %\NOTE{for each $i \in V$} %\myedit{Where did counter came from, client should not store it}
				%\If{Operation is Add/Update/Replace}
				\State Set $\mat{\II}[{x_i},j]\as1$ for $1\le i \le t$, where $x_i$ is index of $w_i$ in $\TW$
				\State Encrypt $f_j$ as $ c_j  \gets \Enc{\kf}{\f_{j}}$
				%\EndIf
				%	\State Set $\I[*,j].st = 1 $ 
				\State Encrypt each row $\mat{\II}[i,j]$ with row keys $r_i$, for $1 \le i \le \NumOfWords$ %\NOTE{and file index $j$???}
				%\State Set $v_i = 0$ for each $i \in V$
				\State Let $\vec{u} \gets (u_1,\dots,u_\NumOfFiles)$, where each $u_i$ is encrypted with $k_3$
				\State Send $(\mat{\II}[*,j], c_j, j, \vec{u})$ to server
				%\end{algorithmic}
				%	\algrule
				%\begin{algorithmic}[1]
				%	\Statex \hspace*{-1.8em}\underline{$(\I,\cib) \as \MainUpdate(\I,\cib,\mat{\II}, c, j)$}
				
				\noindent \hspace{-1.8em} \textbf{Server: } On receive $(\mat{\II}[*,j], c_j, j, \vec{u})$:
				
				\State $\TW[i].u \gets u_i$ and set $\TW[i].v \gets 1$ for $1 \le i \le \NumOfWords$
				\State  Set $\I[*,j]\as\mat{\II}[*,j] $ and $\I[*,j].\st\as 1$ %, for $ 1 \le i \le \NumOfWords $ %and  $0 \le j \le \NumOfFiles $ \NOTE{We might discuss this but all the revealed row keys are updated so I think state should be set to 1 for all matrix}
				%	\State $\TF[j].\ctht$ $\as \TF[j].\ctht+1$
				%\State Update $\cib$ with $c_j$
				%\If {c is $NULL$}
				\State \Return $(\I',\cib',\sigma')$, where $\I' = \I$ with column $j$ updated, $\cib' = \cib$ updated with $c_j$, $\sigma' = \TW $ with counters and states updated % \gets \cib \cup \{(c,j)\}$ 
				%\Else
				%\State \Return $(\I,\cib',\sigma')$, $\cib' \gets \cib \setminus \{(c,j)\}$ 
				%\EndIf
				
			\end{algorithmic}
	}}
\vspace{-3mm}
\end{figure}

% \NOTE{}
% Row counters are increased if the row key was revealed to the server (i.e. last operation on the cell was search). Revealed row keys are re-generated and the column is encrypted with these keys. 
 
% Encrypted 
% 
% column is sent along with the ciphertext of file and the encrypted row indexes. Server only adds the new file to the database (or extract if operation is delete), updates the column j in encrypted matrix and updates the encrypted counter in $\TW$.


%\NOTE{Present according to intuitive step-by-step instruction style, like the one that I gave in the Search, but be GENERAL! For example, Given a file to be updated $ f $ -> extract keywords to be updated-> create unecencrypted column, get the row counter of these keywords from hash table TW from the server -> increase the counter -> generate row keys -> encrypt the column with these keys -> send it along with the ciphertext of file to server, and sends all encrypted updated row counters to server -> server update the column j and the encrypted counter in $ TW $. }




%Moreover, client increases the counter for row key generation and encrypts the column for incident matrix with new row keys (if the key was seen by server in a previous search query) to preserve forward security. Server just replaces the jth column of the incident matrix with the column in token, and adds/deletes the encrypted file to/from the database.


%Note that row keys are updated with the invocation of Update algorithm to provide forward security. %However, as search operation reveals the key, there is no need to increase the counter and change the row keys.



%\begin{scheme}{1}{!b}
%	\floatname{algorithm}{Proposed Scheme}
%	\caption{$ DSSE $ scheme}\label{scheme:DSSE}
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$\K \as \MainGen(1^{\kappa})$}
%		\State $ \kf\as\Kg{1^{\kappa}} $ and $(\kt)\Ra\zo^{\kappa}$
%		%\State $\K\as\{\kf,\kt,\kd\}$
%		\State \Return $ \K $, where $ \K\as\{\kf,\kt\} $ 
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$\f \gets \MainSSEDec_{\K}{(c)}$}
%		\State $\f\as\Dec{\kf}{c,y||\ct}$ %where $u$ is the file counter and $y$ is column index
%		\State \Return $ \f$
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(\I,\cib) \gets \MainSSEEnc_{\K}(\fb)$}
%		\State Extract keywords $(\w_1,\ldots,\w_{\NumOfWords'})$ from files $\fb=\{\f_{id_1},\ldots,\f_{id_{\NumOfFiles'}}\}$
%		\State Add all keywords to hash table $\TW$
%		\State Set $\I[i,j] \as 1$ where $i$ is the index of keywords in $\TW$ and $0 \le j \le \NumOfFiles $ if $\f_j$ contains keyword $i$
%		\State Generate row keys $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $i=1,\ldots,\NumOfWords$
%		\State Encrypt each row of $\I$ with row key $r_i$ %as $\I[i,j]\as \delta[i,j] \xor \HH{r_i||j||\ct_j}$ for $i=1,\ldots,\NumOfWords$ and  $j=1,\ldots,\NumOfFiles$
%		\State Let $\cib$ be the set of files encrypted by $k_1$
%		\State \Return $(\I,\cib)$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(i,r_i) \gets \MainSrchToken{(\K,\w)}$}
%		\State Get the index $i$ for the keyword from $\TW$
%		\State Generate the search token for the keyword with index $i$, $r_i\as \mathsf{PRF}(\kt||i||u_i)$ 
%		\State \Return $(i,r_i)$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$ (D[i], \cib_w) \as \MainSearch((i,r_i),\gamma) $}
%		\If{It is the 1st search on $i$}
%		\State Decrypt $\I[i,*]$ with the key $r_i$
%		\State Let $\I'[i,*]$ be the decryption of $\I[i,*]$
%		\State $D[i] \as \{j: \I'[i,j]=1\}$
%		\State Encrypt $D[i]$ with row key $r_i$
%		\Else
%		\State Decrypt $\I[i,j]$ such that $\I[i,j].st = 1$
%		\State Let $\I'[i,j]$ be the decryption of $\I[i,j]$
%		\State Decrypt $D[i]$ with row key $r_i$
%		\State Add $j$ to $D[i]$ if $\I'[i,j] = 1$
%		\State Delete $j$ from $D[i]$ if $\I'[i,j] \neq 1$
%		\State Re-Encrypt $D[i]$ with row key $r_i$
%		\EndIf
%		
%		%	\State Check if there is a stored $\idw$ for row id $i$ 
%		%	
%		%	\If {$|\idw| \neq 0$}
%		%	
%		%	\If {$\I[i,j].\st = 1$ for $j=1,\ldots,\NumOfFiles$}
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 1$ and j is not in $\idw$}
%		%	\State Add j to $\idw$
%		%	\EndIf
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 0$ and j is in $\idw$}
%		%	\State Extract j from $\idw$
%		%	\EndIf
%		%	\State Set $\I[i,j].\st \as 0$
%		%	\EndIf
%		%	\EndIf
%		%	\If {$|\idw| = 0$ (first search on keywords $w$)}
%		%	\If {$\I[i,j] \xor H(r_i||j||\ct_j) = 1$ for $j=1,\ldots,\NumOfFiles$}
%		%	\State Add j to $\idw$
%		%	\EndIf
%		%	\EndIf
%		\State Set $\cib_w$ as encrypted files corresp. to the indexes in $D[i]$
%		\State \Return $ (D[i],\cib_w) $ (Send to client)
%	\end{algorithmic}
%	%	\algrule
%	
%	
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em} \underline{$(\mat{\II}, c, j)\as \MainUpdateToken(\K,f_j)$}
%		%\State \myedit{Identify the changed cells and increase the counter for them only, at least for update} 
%		\State Set $\mat{\II}[*,j]\as0$ and $c \as NULL$
%		\If{Operation is Add/Update/Replace}
%		\State Extract keywords $(w_1,\ldots,w_t)$ from file $\f_{j}$
%		\State Increase the row counter $u_i$ by 1 and re-generate all row keys  $r_i \as \mathsf{PRF}(\kt||i||u_i)$ for $i=1,\ldots,\NumOfWords$
%		\State Set $\mat{\II}[x_i,j]\as1$ for $i=1,\ldots,t$
%		\State Encrypt the file as $c \gets \Enc{\kf}{\f_{id},j||\ct_j}$
%		\EndIf
%		\State Encrypt $\mat{\II}$ with row key $r_i$
%		\State \Return $\mat{\II}, c, j$ (Send to server)
%	\end{algorithmic}
%	%	\algrule
%	\begin{algorithmic}[1]
%		\Statex \hspace*{-1.8em}\underline{$(\I,\cib) \as \MainUpdate(\I,\cib,\mat{\II}, c, j)$}
%		\State  Set $\I[i,j]\as\mat{\II}[i,j] $ and $\I[i,j].\st\as 1$, for $ 1 \le i \le \NumOfWords $
%		%	\State $\TF[j].\ctht$ $\as \TF[j].\ctht+1$
%		\If {c is $NULL$}
%		\State \Return $(\I,\cib)$, $\cib' \gets \cib \cup \{(c,j)\}$ (Send to client)
%		\Else
%		\State \Return $(\I,\cib)$, $\cib' \gets \cib \setminus \{(c,j)\}$ (Send to client)
%		\EndIf
%		
%	\end{algorithmic}
%\end{scheme}






